Computing linear sections of varieties: quantum entanglement, tensor decompositions and beyond

We study the problem of finding elements in the intersection of an arbitrary conic variety in $\mathbb{F}^n$ with a given linear subspace (where $\mathbb{F}$ can be the real or complex field). This problem captures a rich family of algorithmic problems under different choices of the variety. The special case of the variety consisting of rank-1 matrices already has strong connections to central problems in different areas like quantum information theory and tensor decompositions. This problem is known to be NP-hard in the worst case, even for the variety of rank-1 matrices. Surprisingly, despite these hardness results we develop an algorithm that solves this problem efficiently for "typical" subspaces. Here, the subspace $U \subseteq \mathbb{F}^n$ is chosen generically of a certain dimension, potentially with some generic elements of the variety contained in it. Our main result is a guarantee that our algorithm recovers all the elements of $U$ that lie in the variety, under some mild non-degeneracy assumptions on the variety. As corollaries, we obtain the following new results: $\bullet$ Polynomial time algorithms for several entangled subspaces problems in quantum entanglement, including determining r-entanglement, complete entanglement, and genuine entanglement of a subspace. While all of these problems are NP-hard in the worst case, our algorithm solves them in polynomial time for generic subspaces of dimension up to a constant multiple of the maximum possible. $\bullet$ Uniqueness results and polynomial time algorithmic guarantees for generic instances of a broad class of low-rank decomposition problems that go beyond tensor decompositions. Here, we recover a decomposition of the form $\sum_{i=1}^R v_i \otimes w_i$, where the $v_i$ are elements of the variety $X$. This implies new uniqueness results and genericity guarantees even in the special case of tensor decompositions.

==> newproof.tex <==


%---------------------------------------------------------------------------------------------------%
\section{Algorithm guarantee for generically chosen linear subspaces trivially intersecting $\X$}\label{sec:cert}
%---------------------------------------------------------------------------------------------------%



In this section, we prove the $s=0$ case of Theorem~\ref{thm:intro:intersection}, which informally says that if $R$ is small enough then a generically chosen linear subspace $\U \subseteq \V$ of dimension $R$ is certified by Algorithm~1 as trivially intersecting $\X$. 
% For the lossy proof
% It will be convenient to identify  any operator $\Phi: S^d(\V) \to \field^p$ with the corresponding operator $\Phi \circ P^{\vee}_{\V,d} :\V^{\otimes d} \to \field^p$.
We require the following lemma, which gives a lower bound on the dimension of a contraction with a generically chosen vector. %. %We now state and prove the claim about a lower bound on the dimension for contracting along generic directions, 
%that will be useful in the inductive argument.  


%\newcommand{\hookf}[1]{f^{\otimes \ell} \hook \U}
% \hook{f}{\U}

In what follows, for an element of a symmetric tensor product space $u \in S^d(\V)$, an integer $\ell \in [d-1]$, and a vector $v \in \V$, we define $v^{\otimes \ell} \hook u \in S^{d-\ell}(\V)$ to be the contraction of $u$ with $v^{\otimes \ell}$ in any $\ell$ of the $d$ factors. (The output will be the same regardless of which $\ell$ factors are chosen. We will pick the first $\ell$ factors for concreteness.)


\begin{lemma}\label{lemma:generic_hook:new}
Let $n\in \natural$ be a positive integer, let $d \geq 2$ be an integer, let $\ell \in [d-1]$, let $\X \subseteq \V = \field^n$ be an irreducible variety that is non-degenerate of order $d-1$, and let $\U \subseteq S^d(\V)$ be a linear subspace. Then for a generically chosen vector $v \in \X$, it holds  that $v^{\otimes \ell} \hook \U \subseteq S^{d-\ell}(\V)$, and
\ba\label{eq:generic_hook}
\dim(v^{\otimes \ell}\hook \U)\geq \frac{1}{\binom{n+\ell-1}{\ell}} \cdot \dim(\U).
\ea
\end{lemma}

% \begin{lemma}\label{lem:induction-dim}
% Consider any subspace $\U \subseteq \field^{n_1} \otimes \field^{n_2}$ of dimension $m > (D-1) \times n_1$ for some $D \in \natural_{\ge 1}$, and let the rows of $U \in \field^{m \times (n_1 n_2)}$ represent an orthonormal basis for the subspace. For a generic $x$, the $\text{rank}(U_{(x,1)}) \ge D$ with probability $1$. %Moreover if $\U \in P^{\vee}_{\F^n,d}(\V^{\otimes d})$ 
% % Furthermore when $\field=\real$, for an arbitrary $x \in \real^{n_1}$ with $\|x\|_2 \le \lambda$ and let $\tilde{x} = x + \zeta$ where $\zeta \sim N(0,\rho^2)^n_1$. Then for some universal constants $c_1, c_2, c_3>0$, we have  
% % \begin{equation}
% %     \Pr\Big[\sigma_D\Big( U_{(\tilde{x},1)} \Big) \ge c_1 \rho^{c_3}\Big] \ge 1-\exp(-c_1 n).
% % \end{equation}
% \end{lemma}
%\anote{Need to modify the following proof appropriately.}
\begin{proof}
The fact that $v^{\otimes \ell} \hook \U \subseteq S^{d-\ell}(\V)$ is obvious, so it suffices to prove the dimension bound. Since the set of $v \in \X$ that satisfy~\eqref{eq:generic_hook} is clearly Zariski open, it suffices prove that it is non-empty, i.e. that there exists a single $v \in \X$ that satisfies~\eqref{eq:generic_hook}. Since $\X$ is non-degenerate of order $d-1$, there exists $v_1,\dots, v_{m} \in \X$, where $m=\binom{n+\ell-1}{\ell}$, for which $\{v_i^{\otimes \ell} : i \in [m]\}$ forms a basis of $S^{\ell}(\V)$. Let $\{u_1,\dots,u_m\} \subseteq S^{\ell}(\V)$ be such that $\ip{v_i^{\otimes \ell}}{u_j}=\delta_{i,j}$. Since $\U \subseteq S^d(\V) \subseteq S^{\ell}(\V) \otimes S^{d-\ell}(\V)$, any element $u \in \U$ can be written as $u=\sum_{i=1}^m u_i \otimes w_i$ for some $w_i \in S^{d-\ell}(\V)$. Furthermore, by construction it holds that $w_i = v_i^{\otimes \ell} \hook u \in v_i^{\otimes \ell} \hook \U$. It follows that
% Let $R=\dim(\U)$, let $\{u_1,\dots, u_R\}\subseteq \U$ be a basis for $\U$, let $\{e_1,\dots, e_n\} \in \V$ be a basis for $\V$, and let $\{f_1,\dots, f_n\} \in \V^*$ be the dual basis. Then
\ba
\U \subseteq \sum_{i=1}^m \spn\{u_i\} \otimes (v_i^{\otimes \ell} \hook \U).
\ea
Thus,
\ba
\dim(\U) \leq \sum_{i=1}^m \dim(v_i^{\otimes \ell} \hook \U),
\ea
so there exists some $i \in [m]$ for which
\ba
\dim(v_i^{\otimes \ell} \hook \U) \geq \frac{1}{\binom{n+\ell-1}{\ell}} \cdot \dim(\U).
\ea
This completes the proof.
% We will view the subspace $\U$ through a matrix $U$ representing a basis for $\U$. Let $n' = n^{d-1}$ and let $m= \dim(\U)$. 
% We will abuse notation and consider $f \in \field^{n}$ and a matrix $U \in \field^{m \times (n n')}$ where the rows of $U$ represent elements of the subspace $\field^{n} \otimes \field^{n'}$,  we let $U_{(f,1)} \in \field^{m \times n'}$ represent the matrix obtained by contracting along vector $f \in \field^{n}$ (along the first mode). In other words, if for $j \in [m]$, $U^{(j)} \in \field^{n n'}$ represents the $j$th row of $U$, and $e_1, \dots, e_{n'} \in \field^{n'}$ represent the standard basis vectors then 
% \begin{equation}\label{eq:contraction}
%     U^{(j)}_{(f,1)} = \sum_{i=1}^{n'} \langle U^{(j)}, f \otimes e_i \rangle e_i.
% \end{equation}
%
% Note that when $U$ corresponds to a basis of $\U \subseteq \V^{\otimes d}$, we have $n' = n^{d-1}$, and $U_{(f,1)}$ exactly corresponds to vectors in $\hookfU$. 
% Let $\hat{e}_1, \dots, \hat{e}_{n_1}$ denote the standard basis vectors for $\field^{n}$, and let for each $i \in [n]$, denote by $V_i \coloneqq U_{(e_i,1)}$. 
% %$$\mathcal{V}_i=\text{row-span}(U_{(e_i,1)}) = \span\Big(\Big\{U^{j}_{(e_i,1)}\Big\}\Big). $$
% The columns of $V_1, \dots, V_{n}$ form a partition of the columns of $U$. Hence 
% \begin{equation} \label{eq:induct:rank:add}
% \sum_{i=1}^{n} \rank(V_i) \ge \rank(U) = \dim(\U). 
% \end{equation}
% Hence, there exists an $i^* \in [n]$ such that $V_{i^*}=U_{(e_{i^*}, 1)}$ has rank at least $D=\dim(\U)/n$. By considering the polynomial for the rank-$D$ determinantal variety we get that $\rank(U_{(f,1)})\ge \dim(\U)/n$ for a generic $f$. This proves the lemma. 
\end{proof}


\begin{theorem}\label{thm:generic_cert:new}
Let $\V=\field^n$. For positive integers $d,p$ let
\ba
\Phi: \V^{\otimes d} \to \field^p
\ea
be a linear map that is invariant under permutations of the $d$ subsystems, i.e. $\Phi \circ P_{\V,d}^{\vee}=\Phi$ (where $P_{\V,d}^{\vee}$ is the projection onto the symmetric subspace of $\V^{\otimes d}$). Let $\X_1,\dots, \X_{R} \subseteq \V$ be conic varieties that are non-degenerate of order $d$. If
\begin{equation} \label{eq:ranklb}
    \rank(\Phi) \geq R (d-1)! \binom{n+d-2}{d-1} ,
%    D+ R \cdot \binom{N+d-2}{d-1}  < \binom{N+d-1}{d},
\end{equation}
%\anote{Need to adjust the above bound appropriately}
then for a generic choice of $v_1 \in \X_1, \dots, v_{R} \in \X_{R}$ it holds  that
\begin{equation} \label{eq:setofvectors2:new}
%\{\psi_1, \dots, \psi_D\} \cup
\Big\{\Phi(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d} \Big\}
\end{equation}
is linearly independent.
\end{theorem}


% \begin{theorem}\label{thm:generic_cert}
% Let $\V$ be an $\field$-vector space of dimension $n$, and for positive integers $d,p$ let
% \ba
% \Phi: \V^{\otimes d} \to \field^p
% \ea
% be a linear map.
% Let $\X_1,\dots, \X_{R} \subseteq \V$ be conic varieties that are non-degenerate of order $d$. If
% \begin{equation}
%     \rank(\Phi) \geq R \cdot d n^{d-1},
% %    D+ R \cdot \binom{N+d-2}{d-1}  < \binom{N+d-1}{d},
% \end{equation}
% then for a generic choice of $v_1 \in \X_1, \dots, v_{R} \in \X_{R}$ it holds  that
% \begin{equation} \label{eq:setofvectors2}
% %\{\psi_1, \dots, \psi_D\} \cup
% \Big\{\Phi(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d} \Big\}
% \end{equation}
% is linearly independent.
% \end{theorem}

First note that it suffices to prove Theorem~\ref{thm:generic_cert:new} over $\complex$. Indeed, if $\field=\real$ then we can consider $\real^n$ as a subset of $\complex^n$ and let $\T_1,\dots, \T_R$ be the Zariski closures of $\X_1,\dots, \X_R$ in $\complex^n$. It is clear that $\T_i \cap \real^n=\X_i$ for each $i \in [R]$. Since each $\X_i\subseteq \real^n$ is non-degenerate of order $d$, it follows that each $\T_i\subseteq \complex^n$ is non-degenerate of order $d$. We can similarly view $\Phi$ as a linear map over $\complex$ (the rank of $\Phi$ will not change). Furthermore, $\T:=\T_1 \times \dots \times \T_R$ is the Zariski closure of $\X:=\X_1 \times \dots \times \X_R$. For any Zariski open dense subset $\A \subseteq \T$ for which~\eqref{eq:setofvectors2:new} is linearly independent, it follows from Fact~\ref{fact:real_vs_complex} that $\A \cap \X \subseteq \X$ is a Zariski open dense subset for which~\eqref{eq:setofvectors2:new} is linearly independent. We can therefore assume $\field=\complex$ without loss of generality.



%By Statement~4 of Fact~\ref{fact:real_vs_complex}, for any Zariski open dense subset $\A \subseteq \T_1 \times \dots \times \T_R$ on which~\eqref{eq:setofvectors2:new} is linearly independent, it also holds that $\A^{\real} \subseteq \X_1 \times \dots \times \X_R$ is a Zariski open dense subset on which~\eqref{eq:setofvectors2:new} is linearly independent. We therefore assume $\field=\complex$ without loss of generality.
 
%
% for which $\T_1^{\real}=\X_1, \dots, \T_R^{\real}=\X_R$. Since $\X_1,\dots, \X_R$ are all non-degenerate of order $d$, then each $\T_i$ is also non-degenerate of order $d$. We can similarly view $\Phi$ as a linear map over $\complex$ (the rank of $\Phi$ will not change). By Statement~4 of Fact~\ref{fact:real_vs_complex}, for any Zariski open dense subset $\A \subseteq \T_1 \times \dots \times \T_R$ on which~\eqref{eq:setofvectors2:new} is linearly independent, it also holds that $\A^{\real} \subseteq \X_1 \times \dots \times \X_R$ is a Zariski open dense subset on which~\eqref{eq:setofvectors2:new} is linearly independent. We therefore assume $\field=\complex$ without loss of generality.

To prove Theorem~\ref{thm:generic_cert:new}, we will first define a total ordering of all the index tuples $(a_1, \dots, a_d) \in [R]^{\vee d}$ (recall that $(a_1, \dots, a_d) \in [R]^{\vee d}$ implies $1 \le a_1 \le a_2 \le \dots \le a_d \le R$). 

\begin{definition}\label{def:ordering}
Given two index tuples $(a_1, \dots, a_d), (b_1, \dots, b_d) \in [R]^{\vee d}$, we use the following two rules to determine if $(a_1, \dots, a_d) \prec (b_1, \dots, b_d)$:
\begin{enumerate}
    \item $|\{a_1, \dots, a_d\}|> |\{b_1, \dots, b_d\}|$ i.e., $(a_1, \dots, a_d)$ has more distinct indices than $(b_1, \dots, b_d)$
    \item when $|\{a_1, \dots, a_d\}|= |\{b_1, \dots, b_d\}|$, we go by the the standard lexicographic ordering. For example, $(1,1,2) \prec (1,1,3) \prec \dots \prec (1,1,R) \prec (1,2,1) \dots \prec (R,R,R-1) $. 
\end{enumerate}

\end{definition}

To show that the set of vectors in ~\eqref{eq:setofvectors2:new} is linearly independent, we consider the total ordering of these vectors given by the relation in Definition~\ref{def:ordering}. % and prove that for every $\Phi(v_{i_1} \otimes \dots \otimes v_{i_d})$ is linearly independent $\{\Phi(v_{a_1} \otimes \dots \otimes v_{a_d}): \}$. 
Theorem~\ref{thm:generic_cert:new} is immediate from the following proposition.

\begin{prop}\label{prop:newproof}
Suppose that $\field=\complex$ and the assumptions of Theorem~\ref{thm:generic_cert:new} hold. Then for generically chosen $v_1 \in \X_1,\dots, v_R \in \X_R$ it holds that
\ba\label{eq:prop:newproof}
\Phi(v_{i_1} \otimes \dots \otimes v_{i_d}) \notin \spn\Big\{ \Phi(v_{a_1} \otimes \dots \otimes v_{a_d}): (i_1, \dots, i_d) \succ (a_1, \dots, a_d) \in [R]^{\vee d} \Big\}
\ea
for all $(i_1, \dots, i_d) \in [R]^{\vee d}$.
\end{prop}
To see why this proposition implies Theorem~\ref{thm:generic_cert:new}, simply take the intersection of the Zariski open dense subsets of $\X_1\times \dots \times \X_R$ satisifying~\eqref{eq:prop:newproof} for each $(i_1, \dots, i_d) \in [R]^{\vee d}$. This intersection is again Zariski open dense in $\X_1\times \dots \times \X_R$, and~\eqref{eq:setofvectors2:new} is linearly independent for every tuple in this intersection.
\begin{proof}

For each $i \in [R]$, let $\X_{i,1},\dots, \X_{i,q_{i}}$ be the irreducible components of $\X_i$. Then the irreducible components of $\X_1 \times \dots \times \X_{R}$ are $\X_{1,j_1} \times \dots \times \X_{R,j_{R}}$ as $j_1,\dots, j_{R}$ range over $[q_1],\dots, [q_{R}]$, respectively. It suffices to prove that~\eqref{eq:prop:newproof} holds on a Zariski open dense subset of each component. To ease notation, we redefine $\X_1=\X_{1,j_1}$, \dots, $\X_R=\X_{R,j_R}$, and prove that $~\eqref{eq:prop:newproof}$ holds on a Zariski open dense subset of $\X_1 \times \dots \times \X_{R}$. We prove this by induction on $d$, starting with the base case $d=1$.

\paragraph{Base case ($d=1$).}
We will prove the stronger statement that $\{\Phi(v_1),\dots, \Phi(v_R)\}$ is linearly independent for generically chosen $v_1 \in \X_1, \dots, v_R \in \X_R$. Since linear independence of $\{\Phi(v_1),\dots, \Phi(v_R)\}$ is an open condition on $\X_1\times \dots \times \X_R$, it suffices to prove that there exists $v_1\in \X_1,\dots, v_R \in \X_R$ for which linear independence holds. By assumption, for each $i \in [R]$ it holds that $\spn(\X_{i})=\V$. Let $\U_0=\ker(\Phi)$. Since $\dim(\U_0) \leq n-R < n$, it holds that $\ker(\Phi) \cap \X_{1} \subseteq \X_{1}$ is a proper Zariski closed subset of $\X_{1}$. It follows that for any
\ba
v_1 \in \A_{1}:= \X_{1}\setminus (\ker(\Phi) \cap \X_{1}),
\ea
we have $\U_0 \cap \spn\{v_1\}=\{0\}$. If $R=1$ then we are done, as $\U_0 \cap \spn\{v_1\}=\{0\}$ is equivalent to the singleton $\{\Phi(v_1)\}$ being linearly independent in this case. Otherwise, fix any vector $v_1 \in \A_{1}$, and let $\U_{1}=\U_0+ \spn\{v_1\}$. Since ${\dim(\U_{1}) \leq n-R+1 < n}$, there similarly exists a Zariski open dense subset $\A_{2} \subseteq \X_{2}$ such that for all $v_2 \in \A_{2}$ it holds that $\U_{1} \cap \spn\{v_2\} = \{0\}$. If $R=2$ then we are done, as the set is linearly independent if and only if $\U_0 \cap \spn\{v_1\}=\{0\}$ and ${\U_{1} \cap \spn\{v_2\} = \{0\}}$. Otherwise, fix any vector $v_2 \in \A_{2}$, and let $\U_2=\U_1 + \spn\{v_2\}$. Continuing in this way inductively, for each $i \in \{2,\dots, R\}$ let $\U_i=\U_{i-1}+\spn\{v_{i}\}$, where $v_{i}\in \X_{i}$ is any vector for which $\U_{i-1} \cap \spn\{v_{i}\}=\{0\}$ (which is guaranteed to exist since ${\dim(\U_{i-1}) \leq n-R+{i-1} < n}$ for all $i \in [R]$). In the end, we have constructed a tuple $(v_1,\dots, v_{R})\in \X_{1}\times \dots \times \X_{R}$ for which the set $\{\Phi(v_1),\dots, \Phi(v_R)\}$ is linearly independent. This completes the proof of the base case $d=1$.

\paragraph{Inductive proof ($d>1$).} Proceeding inductively, suppose $d>1$. For each $I=(i_1,\dots,i_d)\in [R]^{\vee d}$, let
\ba
\trouble(I)=\Big\{ a \in [R]^{\vee d}~:~ \{a_1, \dots, a_d \} = \{i_1,\dots, i_d\} \text{ and } (a_1, \dots, a_d) \prec (i_1, \dots, i_d) \Big\},
\ea
where $\prec$ is defined in Definition~\ref{def:ordering}.
%Finally, let $G=G_1\cup \dots \cup G_d$. Note that the set~\eqref{eq:setofvectors1} is linearly independent if and only if $G$ is linearly independent and $\left[\ker(\Phi)\cap S^d(\V)\right] \cap \spn\{G\}=\{0\}$. In turn, this is equivalent to the statement that for all $k \in [d]$ and $I=(i_1,\dots, i_d)\in [R]^{\vee d}$ with $\abs{I}=k$, it holds that $T(I)$ is linearly independent and
%\ba\label{eq:lininequiv}
%T(I) \cap \left[ \left[\ker(\Phi)\cap S^d(\V)\right] + \spn\left\{\bigcup_{k' \in [k-1]} G_{k'} \setminus T(I)\right\}\right]=\{0\}.
%\ea
%$\trouble(I)$ corresponds to all those terms where the indic
Here $\{a_1, \dots, a_d\}=\{i_1, \dots, i_d\}$ means the distinct indices involved in the term corresponding to $a_1, \dots, a_d$ are exactly the distinct indices among $i_1, \dots, i_d$ (note that some may be repeated).\footnote{Here, $T(I)$ represents the set of the vectors that will be ``troublesome'' for $v_{i_1}\otimes \dots \otimes v_{i_d}$ because they are composed of the same underlying vectors $v_{i_1}, \dots, v_{i_d}$. }  

%Finally, let $G_{d+1}$ be a basis of $\ker(\Phi)\cap S^d(\V)$, and let $G=G_1 \cup \dots \cup G_d \cup G_{d+1}$. Note that the set~\eqref{eq:setofvectors1} is linearly independent if and only if $G$ is linearly independent.
Let $w_1 \vee \dots \vee w_d = P^{\vee}_{\V,d} (w_1 \otimes \dots \otimes w_d)$ when $d$ is a positive integer and $w_1,\dots, w_d \in \V$. Note that since $\Phi=\Phi \circ P^{\vee}_{\V,d},$ we have $\Phi(w_1 \otimes \dots \otimes w_d)=\Phi(w_1 \vee \dots \vee w_d)$ for all $w_1,\dots, w_d \in \V$. The proposition is equivalent to the following claim:

\begin{claim} It holds that
\begin{align}
\Pi^{\perp}_{\prec I} \big(v_{i_1} \vee \dots \vee v_{i_d}\big) \notin \spn\{ \Pi^{\perp}_{\prec I} (v_{a_1}\vee \dots \vee v_{a_d}) : a \in \trouble(I) \}\label{eq:claim:higherorder2:new}  %\\
%\Pi^{\perp}_{<I}  \text{ is the projector perpendicular to }  &\text{span}\big(\big \cup_{k' \le k} G_{k'} \setminus \trouble(I)  \big)
%P^{\vee}_{\V,d}\Big(v_{i_1} \otimes v_{i_2} \otimes \dots \otimes v_{i_d}\Big) \notin \text{span}\Big(\Big\{ P^{\vee}_{\V,d}(v_{a_1} \otimes \dots \otimes v_{a_d}) ~:~ |\{ a_1, \dots, a_d\}| \le |\{i_1, \dots, i_d\}| \Big\}\Big),
\end{align}
 for generically chosen $v_1\in \X_1,\dots, v_{R} \in \X_{R}$, where $\Pi_{\prec I}^{\perp}$ is the orthogonal projection onto the subspace of $S^d(\V)$ orthogonal to
 \ba\label{eq:im_pi_I1}
\Z_I:=\ker(\Phi)\cap S^d(\V) + \spn\{v_{a_1} \vee \dots \vee v_{a_d}: a \in [R]^{\vee d}\setminus \trouble(I) \quad \text{and} \quad (i_1, \dots, i_d) \succ (a_1, \dots, a_d)\}.
 \ea
 \end{claim}
 
%To see why the claim implies the proposition, note that
%\ba
%\ker(\Phi)\cap S^d(\V) + \{v_{a_1} \vee \dots \vee v_{a_d}: (i_1, \dots, i_d) \succ (a_1, \dots, a_d) \in [R]^{\vee d} \} \subseteq \ker(\Pi_{\prec I}^{\perp}) \cup P^{\vee}_{\V,d}
%\ea
To see why the claim is equivalent, note that~\eqref{eq:prop:newproof} holds if and only if
\ba
v_{i_1} \vee \dots \vee v_{i_d} \notin \spn\{v_{a_1}\vee \dots \vee v_{a_d} : (i_1,\dots, i_d) \succ (a_1,\dots, a_d) \in [R]^{\vee d}\} + \ker(\Phi)\cap S^d(\V),
\ea
and~\eqref{eq:im_pi_I1} holds if and only if
\ba
v_{i_1} \vee \dots \vee v_{i_d} \notin \spn\{v_{a_1}\vee & \dots \vee v_{a_d} : a \in T(I)\} + \Z_I.
\ea
The righthand sides of these expressions are equal.

%we can order all the vectors in $G$ in any order with the vectors in $G_{d+1}$ first, followed by those in $G_d$, and so on, until $G_1$. The above claim implies that each vector in this sequence is not contained in the span of the vectors before it, so $G$ is linearly independent. \\
%Indeed, suppose that
%Indeed, suppose that $\left[\ker(\Phi)\cap S^d(\V)\right] \cap \spn\{G\}=\{0\}$. For each $k \in [d]$ fix any ordering of the set of tuples $I=(i_1,\dots, i_d)\in [R]^{\vee d}$ for which $\abs{I}=k$, choose the minimal $k\in [d]$, for which there exists $I \in [R]^{\vee d}$ for which~\eqref{eq:lininequiv} does not hold. Then there exists $u \in \trouble(I), v \in \ker(\Phi)\cap S^d(\V), w\in \spn\left\{\bigcup_{k' \in [k-1]} G_{k'} \setminus \trouble(I)\right\}$ for which $u=v+w$.
%\begin{claim}
%\textit{For all $k \in [d]$ and $I=(i_1,\dots, i_d)\in [R]^{\vee d}$ with $\abs{I}=k$, for generic $v_1,\dots, v_{R} \in \V$ it holds that $\trouble(I)$ is linearly independent and
%\ba
%\trouble(I) \cap \left[ \left[\ker(\Phi)\cap S^d(\V)\right] + \spn\left\{\bigcup_{k' \in [k-1]} G_{k'} \setminus \trouble(I)\right\}\right]=\{0\}.
%\ea}
%\end{claim}
%Indeed, if $G$ is linearly independent and $\left[\ker(\Phi)\cap S^d(\V)\right] \cap \spn\{G\}=\{0\}$, then it is clearly the case that
To complete the proof, we prove the claim. For each choice of vectors $v_1\in \X_1,\dots, v_R \in \X_R$, and each $a \in [R]$, $d \in \mathbb{N}$, let
\ba
\U_a^{(d)}=P_{\V,d}^{\vee}(\spn\{v_a\} \otimes \V^{\otimes d-1}).
\ea
For each $I=(i_1,\dots, i_d)\in [R]^{\vee d}$, let
\ba
\U_{-I}=\ker(\Phi)\cap S^d(\V) + \spn\bigg\{\bigcup_{a \in [R]\setminus \{i_1,\dots, i_d\}} \U_a^{(d)} \bigg\}.
\ea
Then $\dim(\U_a^{(d)}) \leq \binom{n+d-2}{d-1}$ and
% \ba
% \U_a \coloneqq \spn\{v_a\} \otimes \V^{\otimes d-1}+\V \otimes \spn\{v_a\} \otimes \V^{\otimes d-2} +\dots + \V^{\otimes d-1} \otimes \spn\{v_a\}.
% \ea
% For each $I=(i_1,\dots, i_d)\in [R]^{\vee d}$, let
% \ba
% \U_{-I}=\spn\bigg\{G_0 \cup \bigcup_{a \in [R]\setminus \{i_1,\dots, i_d\}} \U_a\bigg\}.
% \ea
% Then $\dim(\U_a)\le d n^{d-1}$, and %\binom{n+d-2}{d-1}$, and
\ba
\dim(\U_{-I})&\leq \dim(\ker(\Phi)\cap S^d(\V))+(R-k) \binom{n+d-2}{d-1} \\
			&=\binom{n+d-1}{d}-\rank(\Phi)+(R-k) \binom{n+d-2}{d-1} \\
			&\le \binom{n+d-1}{d} - k (d-1)! \binom{n+d-2}{d-1} \quad (\text{from }\eqref{eq:ranklb}, \text{ and } (d-1)!\ge 1),
%			&\leq n^d - k d n^{d-1}. %\binom{N+d-1}{d}-k\binom{N+d-2}{d-1}.
\ea
where $k:=|\{i_1,\dots,i_d\}|$.

Let $\tilde{\Pi}^{\perp}_{-I}$ be the orthogonal projection onto $\U_{-I}^{\perp}$, the orthogonal complement of $\U_{-I}$ in $S^d(\V)$.
We make three observations: % about $\U_{-I}$:
\begin{itemize}
    \item[(i)]  $\U_{-I}$ only depends on $\{v_j : j \notin \{i_1, \dots, i_d\}\}$, and is independent of  $v_{i_1}, \dots, v_{i_d}$.
\item[(ii)] $\U_{-I} \supseteq \Z_I$.%Hence $\text{range}(\Pi^\perp_{-I}) \subseteq \text{range}(\Pi^{\perp}_{<I})$.
\item[(iii)] $\text{rank}(\tilde{\Pi}^\perp_{-I}) = \binom{n+d-1}{d} - \dim(\U_{-I}) \ge k (d-1)! \binom{n+d-2}{d-1}$.
%$\rank(\Phi)-(R-k) \binom{n+d-2}{d-1} \ge k \binom{n+d-2}{d-1}$. %$\ge \rank(\Phi)-(R-k)d n^{d-1}\geq k \cdot d n^{d-1}.$
\end{itemize}
By observation (ii), to establish the claim it suffices to prove that for generically chosen $v_1\in \X_1,\dots, v_{R} \in \X_{R}$ it holds that
\begin{align} \label{eq:equiv:higherorder31}
   \tilde{\Pi}^{\perp}_{-I} \big(v_{i_1} \vee \dots \vee v_{i_d}\big) \notin \spn\{ \tilde{\Pi}^{\perp}_{-I} (v_{a_1}\vee \dots \vee v_{a_d}) : (a_1,\dots, a_d) \in \trouble(I) \}.
\end{align}
Using Chevalley's theorem, it is not difficult to show that the set of elements of $\X_1\times \dots \times \X_{R}$ satisfying~\eqref{eq:equiv:higherorder31} is constructible~\cite[Exercise II.3.19]{hartshorne2013algebraic}. Since any constructible set contains an open dense subset of its closure, it suffices to prove that the set~\eqref{eq:equiv:higherorder31} is Zariski dense in $\X_1\times \dots \times \X_{R}$~\cite[Lemma 2.1]{an2012rigid}.
%Let $\U_{-I}^{\perp} \subseteq S^d(\V)$ be the orthogonal complement to $\U_{-I}$ in $S^d(\V)$. Then $\dim(\U_{-I}^{\perp})=\rank(\tilde{\Pi}_{-I}^{\perp})$.
%
%
%
%
%
%\begin{align}
%\U_{-I} \cap \text{span}(\trouble(I)) &= \U_{-I} \cap \text{span}\Big\{(P^{\vee}_{\V,d}(v_{a_1} \otimes \dots \otimes v_{a_d})  : \{a_1, \dots, a_d \} = \{i_1, \dots , i_d\} \Big\} = \{0\}.
%\end{align}

Let $\ell$ denote the largest integer in $[d]$ such that $i_{\ell} = i_1$. By the definition of $\trouble(I)$, for every $(a_1,\dots, a_d) \in \trouble(I)$, we have $a_1 = a_2 = \dots = a_\ell = i_1$ (but $a_{\ell+1}$ may or may not be equal to $i_1$). If $\ell=d$, then $\trouble(I)$ is empty. Since $\X_{i_1}$ is non-degenerate of order $d$, it holds that $\spn\{v^{\otimes d} : v \in \X_{i_1}\}=S^d(\V)$. For any choice of $\{v_j: j \neq i_1\}$, it holds that $\rank(\tilde{\Pi}^{\perp}_{-I}) >0$, so a generic choice of $v_{i_1} \in \X_{i_1}$ satisfies~\eqref{eq:equiv:higherorder3}. In more details, we have demonstrated the existence of a set
\ba\label{eq:zariski_dense}
\bigcup_{(v_1, \dots, v_{\hat{i_1}},\dots, v_d)\in \X_1 \times \dots \times \X_{\hat{i_1}}\times \dots \times \X_d} (v_1,\dots,v_{i_1-1}) \times \A_{v_1, \dots, v_{\hat{i_1}},\dots, v_d} \times (v_{i_1+1}, \dots, v_{d})
\ea
such that~\eqref{eq:equiv:higherorder3} holds for every element, where $\A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \subseteq \X_{i_1}$ is Zariski open dense for every choice of $(v_1,\dots,v_{\hat{i_1}},\dots, v_d)$. The set defined in~\eqref{eq:zariski_dense} is Zariski-dense in $\X_1 \times \dots \times \X_R$. Indeed, for any non-empty Zariski open subset $\C \subseteq \X_1 \times \dots \times \X_R$, $\C$ must intersect some $(v_1,\dots,v_{i_1-1})\times \X_{i_1} \times (v_{i_1+1}, \dots, v_{d})$ in a non-empty open subset. Since $\A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \subseteq \X_{i_1}$ is Zariski open dense, it follows that $\C$ must intersect $(v_1,\dots,v_{i_1-1}) \times \A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \times (v_{i_1+1}, \dots, v_{d})$, and hence it must intersect~\eqref{eq:zariski_dense}. This completes the proof of the case $\ell=d$.

Henceforth we assume $1 \le \ell \le d-1$, and prove the claim by applying the inductive hypothesis with degree $(d-\ell)$. 
%Note that $v_{i_1}$ is chosen generically. 
%\anote{ $v_{i_1}$ is chosen generically from the variety}   
For each choice of $v_{i_1} \in \X_{i_1}$, define a linear map
\ba
\tilde{\Phi}:\V^{\otimes (d-\ell)} \to S^d(\V)
\ea
by $\tilde{\Phi}(u)=\tilde{\Pi}^{\perp}_{-I}(v_{i_1}^{\otimes \ell} \otimes u)$. Then
\ba
\setft{Im}(\tilde{\Phi}^*)=v_{i_1}^{\otimes \ell} \hook \U_{-I}^{\perp},
\ea
and we denote this image by $\W'_{(d-\ell)}$ (recall that $(\cdot)^*$ denotes the conjugate-transpose). By Lemma~\ref{lemma:generic_hook:new}, for generically chosen $v_{i_1} \in \X_{i_1}$ it holds that $\W'_{(d-\ell)} \subseteq S^{d-\ell}(\V)$ and
\ba\label{eq:ranklb:2}
\rank(\tilde{\Phi}) = \dim(\W'_{(d-\ell)}) = \dim\big(v_{i_1}^{\otimes \ell} \hook \U_{-I}^{\perp} \big) \geq \frac{1}{\binom{n+\ell-1}{\ell}} \cdot \dim(\U_{-I}^{\perp}) 
%\ge \frac{\rank(\Phi)-(R-k) \binom{n+d-2}{d-1}}{\binom{n+\ell-1}{\ell}} .
\ge k(d-1)!\cdot \frac{  \binom{n+d-2}{d-1}}{\binom{n+\ell-1}{\ell}} .
\ea
We denote the Zariski open dense subset of $\X_{i_1}$ for which this holds by $\A_{(v_j : j \notin \{i_1,\dots, i_d\})} \subseteq \X_{i_1}$ (the subscript refers to the fact that this set depends only on $\{v_j : j \notin \{i_1,\dots, i_d\}\}$). Let $\W^{\perp}_{(d-\ell)}$ represent the subspace of $\W'_{(d-\ell)}$ that is orthogonal to $\U^{(d-\ell)}_{i_1}$, and let $\Phi_{(d-\ell)}$ be the orthogonal projection onto the subspace $\W^{\perp}_{(d-\ell)}$. Note by our ordering $\prec$, and our definition of $\trouble(I)$, 
\ba\label{eq:newproof:covered11}
    \Big\{ v_{a_{\ell+1}}\vee \dots \vee v_{a_{d}} : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d)\in \trouble(I) \quad \text{and} \quad  a_{\ell+1} = i_1 \Big\} &\subseteq \U^{(d-\ell)}_{i_1},
\ea
    and
    \ba\label{eq:claim:higherorder2:new1}
        \Big\{ v_{a_{\ell+1}}\vee& \dots \vee v_{a_{d}} : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d)\in \trouble(I) \quad \text{and} \quad  a_{\ell+1} \neq i_1 \Big\}\\
        &=\Big\{ v_{a_{\ell+1}} \vee \dots \vee v_{a_{d}} : (a_{\ell+1},\dots, a_d) \in \trouble(i_{\ell+1}, \dots, i_d) \Big\},
        \ea
%    \Big\{ v_{a_1} \otimes \dots \otimes v_{a_{d}}: a\in \trouble(I) \quad \text{and} \quad a_{\ell+1} \ne i_1 \Big\} &= \Big\{ v_{i_1}^{\otimes \ell} \otimes v_{a_{\ell+1}} \otimes \dots \otimes v_{a_{d}} \in \trouble(I) : \{a_{\ell+1},\dots,  a_{d}\} = \{i_{\ell+1}, \dots, i_d\} \Big\}. \label{eq:newproof:covered2}
%\ea
%Moreover for every vector $v_{a_1} \otimes \dots \otimes v_{a_{d}} \in \trouble(I)$ not covered in \eqref{eq:newproof:covered}, we have that $\{a_{\ell+1}, \dots, a_{d} \} = \{i_{\ell+1}, \dots, i_d \}$.  
%Hence Claim A, i.e., \eqref{eq:claim:higherorder2:new}, now follows from the following claim: 
where
   \ba
\trouble(i_{\ell+1}, \dots, i_d)=\Big\{ (a_{\ell+1},\dots, a_d) \in [R]^{\vee (d-\ell)}:& \{a_{\ell+1}, \dots, a_d\}=\{i_{\ell+1}, \dots, i_d\}\\
&\text{and} \; (i_{\ell+1}, \dots, i_d) \succ (a_{\ell+1}, \dots, a_d) \Big\}.
\ea
%}
%Note that $\trouble(i_{\ell+1}, \dots, i_d)$ also contains some extra vectors compared to the ones in \eqref{eq:newproof:covered2} (since it does not impose that $a_1 = i_1, \dots, a_\ell = i_\ell$). \bnote{Does it actually contain extra vectors?}
Note that
\ba
\rank(\Phi_{(d-\ell)}) &= \dim(\W^{\perp}_{(d-\ell)}) \ge \dim(\W'_{(d-\ell)})-\binom{n+d-\ell-2}{d-\ell-1} \\
%&\ge \frac{\rank(\Phi)-(R-k) \binom{n+d-2}{d-1}}{\binom{n+\ell-1}{\ell}} -\binom{n+d-\ell-2}{d-\ell-1} \\
&\ge \frac{k (d-1)! \binom{n+d-2}{d-1} }{\binom{n+\ell-1}{\ell}} -\binom{n+d-\ell-2}{d-\ell-1} \\
&\ge \frac{k (d-1)!}{\binom{d-1}{\ell}} \cdot\binom{n+d-\ell-2}{d-\ell-1} -\binom{n+d-\ell-2}{d-\ell-1}\\
&\ge (k-1) \cdot (d-\ell-1)! \cdot \binom{n+d-\ell-2}{d-\ell-1}.
\ea
The penultimate line follows from $\binom{n+d-2}{d-1} \cdot \binom{d-1}{\ell}\ge \binom{n+d-\ell-2}{d-\ell-1} \cdot \binom{n+\ell-1}{\ell}$.
Furthermore, it holds that
\ba
&\Phi_{(d-\ell)}=\Phi_{(d-\ell)} \circ P^{\vee}_{\V,(d-\ell)},\\
&\trouble(i_{\ell+1}, \dots,i_d)\subseteq (i_{\ell+1},\dots, i_d)^{\vee (d-\ell)},\\
&\abs{\{i_{\ell+1}, \dots,i_d\}}=k-1,
\ea
and the varieties $\X_{i_{\ell+1}},\dots, \X_{i_d}$ are non-degenerate of order $d-\ell$. It follows from the induction hypothesis with degree $(d-\ell)$, $R=k-1$, and the operator $\Phi=\Phi_{(d-\ell)}$ that
\begin{align} \label{eq:equiv:higherorder41}
\Phi_{(d-\ell)} \big(v_{i_{\ell+1}} \vee \dots \vee v_{i_d}\big)\notin \spn\{ \Phi_{(d-\ell)}  (v_{a_{\ell+1}}\vee \dots \vee v_{a_{d}}) : (a_{\ell+1},\dots,a_d) \in \trouble(i_{\ell+1},\dots, i_d ) \}
\end{align} 
for generically chosen $v_{i_{\ell+1}}\in \X_{i_{\ell+1}}\dots, v_{i_d} \in \X_{i_{d}}$. We denote the Zariski open dense subset of $\X_{i_{\ell+1}}\times \dots \times \X_{i_d}$ for which this holds by $\C_{(v_j : j \notin \{i_{\ell+1},\dots, i_d\})}\subseteq \X_{i_{\ell+1}}\times \dots \times \X_{i_d}.$
%Moreover the subspace $\W^{\perp}_{d-\ell}$ corresponding to $\Phi_{d-\ell}$ is also a symmetric subspace. Furthermore, $\trouble(i_{\ell+1}, \dots,i_d) \subset (\spn\{v_{i_{\ell+1}},\dots,v_{i_d}\})^{\otimes d-\ell}$ and $|v_{i_{\ell+1}},\dots,v_{i_d}\}|=k-1$. Also $\Phi_{d-\ell}$ is fixed independent of the generic choices of $v_{i_{\ell+1}},\dots,  v_{i_d}$ (note that $\Phi_{d-\ell}$ may depend on $v_{i_1}$), and  no irreducible component of any of the varieties $\X_1,\dots, \X_{R}$ has equations in degree $d-\ell$.
%%\noindent {\em {\bf Claim B.} For generic $v_1 \in \X_1,\dots, v_{R} \in \X_{R}$, we have    
%We now use the inductive hypothesis i.e., Proposition~\ref{prop:newproof} with degree $(d-\ell)$, $R=k-1$, and the operator $\Phi=\Phi_{d-\ell}$ to conclude 
%\begin{align} \label{eq:equiv:higherorder4}
%   &\Phi_{d-\ell} \big(v_{i_{\ell+1}} \otimes \dots \otimes v_{i_d}\big) \text{ is linearly independent of } \{ \Phi_{d-\ell}  u : u \in \trouble(i_{\ell+1},\dots, i_d ) \}.
%\end{align} 

This establishes~\eqref{eq:equiv:higherorder31} as follows: First, note that~\eqref{eq:equiv:higherorder31} is equivalent to
\begin{align}
   \tilde{\Pi}^{\perp}_{-I} \big(v_{i_1}^{\otimes \ell} \otimes (v_{i_{\ell+1}}\vee \dots \vee v_{i_d})\big) \notin \spn\{ \tilde{\Pi}^{\perp}_{-I} \big((v_{i_1})^{\otimes \ell} \otimes (v_{a_{\ell+1}} \vee \dots \vee v_{a_d})\big) : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d) \in \trouble(I) \}.
\end{align}
Indeed, since $\tilde{\Pi}^{\perp}_{-I}=\tilde{\Pi}^{\perp}_{-I} \circ P^{\vee}_{\V,d}$, it also holds that $\tilde{\Pi}^{\perp}_{-I}=\tilde{\Pi}^{\perp}_{-I} \circ (\mathbb{1}_{\V}^{\otimes \ell} \otimes P^{\vee}_{\V,(d-\ell)})$. By the definition of $\tilde{\Phi}$, this is equivalent to
\begin{align}
   \tilde{\Phi}(v_{i_{\ell+1}}\vee \dots \vee v_{i_d}) \notin \spn\{ \tilde{\Phi}(v_{a_{\ell+1}} \vee \dots \vee v_{a_d}) : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d) \in \trouble(I) \},
\end{align}
i.e.
\begin{align}
v_{i_{\ell+1}}\vee \dots \vee v_{i_d} \notin \spn\{ v_{a_{\ell+1}} \vee \dots \vee v_{a_d} : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d) \in \trouble(I) \} + \ker(\tilde{\Phi}) \cap S^{d-\ell}(\V),\\
\label{eq:right11}
\end{align}
where $\ker(\tilde{\Phi}) \cap S^{d-\ell}(\V)=\im((\tilde{\Phi})^*)^{\perp}\cap S^{d-\ell}(\V)=(W'_{(d-\ell)})^{\perp}\cap S^{d-\ell}(\V).$ Similarly,~\eqref{eq:equiv:higherorder41} is equivalent to
\begin{align}\label{eq:right21}
v_{i_{\ell+1}} \vee \dots \vee v_{i_d} \notin \spn\{ v_{a_{\ell+1}}\vee \dots \vee v_{a_{d}} : (a_{\ell+1},\dots,a_d) \in \trouble(i_{\ell+1},\dots, i_d ) \} + \ker(\Phi_{(d-\ell)}),
\end{align}
where $\ker(\Phi_{(d-\ell)})=\U_{i_1}^{(d-\ell)} + (W'_{(d-\ell)})^{\perp}\cap S^{d-\ell}(\V).$ By~\eqref{eq:newproof:covered11} and~\eqref{eq:claim:higherorder2:new1}, the righthand side of~\eqref{eq:right11} is contained in the righthand side of~\eqref{eq:right21}. Since we have shown that~\eqref{eq:right21} holds generically, it follows that~\eqref{eq:right11} holds generically.

In more details, we have proven that~\eqref{eq:equiv:higherorder31} holds for every tuple in the set
\ba~\label{eq:zariski21}
\bigcup_{\substack{(v_j : j \notin \{i_1,\dots, i_d\}) \in \times_{j \notin \{i_1,\dots, i_d\}} \X_j\\ v_{i_1} \in \A_{(v_j : j \notin \{i_1,\dots, i_d\})}}} (v_j : j \notin \{i_1,\dots, i_d\}) \times (v_{i_1}) \times \C_{(v_j : j \notin \{i_{\ell+1},\dots, i_d\})}.
\ea
To complete the proof, it suffices to prove that~\eqref{eq:zariski21} is Zariski dense in $\X_1 \times \dots \times \X_R$. Let $\D \subseteq \X_1 \times \dots \times \X_R$ be a non-empty open subset. Then there exists $(v_j : j \notin \{i_1,\dots, i_d\}) \in \bigtimes_{j \notin \{i_1,\dots, i_d\}} \X_j$ for which
\ba
\D_1:= \D \cap \left((v_j : j \notin \{i_1,\dots, i_d\}) \times \left(\bigtimes_{j \in \{i_1,\dots, i_d\}} \X_j\right)\right)
\ea
is Zariski open dense in $(v_j : j \notin \{i_1,\dots, i_d\})\times \left(\bigtimes_{j \in \{i_1,\dots, i_d\}} \X_j\right)$. For this choice of $(v_j : j \notin \{i_1,\dots, i_d\})$, there exists $v_{i_1} \in \A_{(v_j : j \notin \{i_1,\dots, i_d\})}$ for which 
\ba
\D_2 := \D_1 \cap \left((v_j : j \notin \{i_{\ell+1},\dots, i_d\}) \times \left(\bigtimes_{j \in \{i_{\ell+1},\dots, i_d\}} \X_j\right)\right)
\ea
is Zariski open dense in $(v_j : j \notin \{i_{\ell+1},\dots, i_d\})\times \left(\bigtimes_{j \in \{i_{\ell+1},\dots, i_d\}} \X_j\right)$. Thus,
\ba
\D_2 \cap \left((v_j : j \notin \{i_{\ell+1},\dots, i_d\}) \times \C_{(v_j : j \notin \{i_{\ell+1},\dots, i_d\})}\right) \neq \emptyset,
\ea
so $\D$ intersects the set defined in~\eqref{eq:zariski21} non-trivially. Since $\D$ was an arbitrary non-empty open subset of $\X_1\times \dots \times \X_R$, it follows that the set~\eqref{eq:zariski21} is Zariski dense in $\X_1 \times \dots \times \X_R$. This completes the proof.
%
%Putting these genericity claims together, this proves the existence of a set similar to~\eqref{eq:zariski_dense}: For each choice of $\{v_j : j \notin \{i_1,\dots, i_d\}\}$, and each corresponding choice of $v_{i_1} \in \A_{(v_j : j \notin \{i_1,\dots, i_d\})}$, there is a Zariski open dense subset $\C_{(v_j : j \notin \{i_{\ell+1},\dots, i_d\})} \subseteq \X_{i_{\ell+1}} \times \dots \times \X_{i_{d}}$ for which~\eqref{eq:equiv:higherorder3} holds. Taking the union of these sets over all choices of linearly independent $\{v_j : j \notin \{i_1,\dots, i_d\}\}$, $v_{i_1} \in \A_{(v_j : j \notin \{i_1,\dots, i_d\})}$, and $(v_{i_{\ell+1}}, \dots, v_{i_d}) \in \C_{(v_j : j \notin \{i_{\ell+1},\dots, i_d\})}$ gives a Zariski dense subset of $\X_1 \times \dots \times \X_R$ on which~\eqref{eq:equiv:higherorder3} holds. Since~\eqref{eq:equiv:higherorder3} holds on a constructible subset of $\X_1\times \dots \times \X_R$, and a constructible set contains a Zariski open dense subset of its closure, this proves that~\eqref{eq:equiv:higherorder3} holds on a Zariski open dense subset of $\X_1\times \dots \times \X_R$.
%\ba\label{eq:zariski_dense2}
%\bigcup_{v\in \B} (v_1,\dots,v_{i_1-1}) \times \A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \times (v_{i_1+1}, \dots, v_{d})
%\ea
%Thus,~\eqref{eq:equiv:higherorder3} holds for generic choices of $v_1 \in \X_1,\dots, v_R \in \X_R$.
%This now implies Claim A (i.e., \eqref{eq:claim:higherorder2:new}) as follows:  by definition, $\Phi' (u) = \tilde{\Pi}^{\perp}_{-I} (v_{i_1}^{\otimes \ell} \otimes u)$, where $\Phi'$ is the projector onto the subspace $\W'_{d-\ell}$ and  $\Phi_{d-\ell}$ is the projector of the $\W^{\perp}_{d-\ell}$ (the subspace of $\W'_{d-\ell}$ that is orthogonal to $\U^{(d-\ell)}_{i_1}$). Also from \eqref{eq:newproof:covered1} and  \eqref{eq:newproof:covered2}, every $v_{a_1} \otimes \dots \otimes v_{a_{d}} \in \trouble(I)$ is either contained in $\{ v_{i_1}^{\otimes \ell} \otimes \U^{(d-\ell)}_{i_1} \cup v_{i_1}^{\otimes \ell} \otimes \trouble(i_{\ell+1}, \dots, i_{d}) \}$. 
%% Since $\abs{\{i_1,\dots, i_d\}}=k$, and
%% \ba
%% \rank \geq \frac{1}{\binom{n+\ell-1}{\ell}} \dim(\U_{-I}^{\perp}) ,
%% \ea
%% it follows from the induction hypothesis that for a generic choice of $v_{i_1}\in \X_{i_1},\dots, v_{i_d}\in \X_{i_d}$ it holds that $(f \hook_1 \U_{-I}^{})\cap (f \hook_1 \spn(\trouble(I)))=\{0\}$. Since $f\in \V^*$ is also generic, this implies $\U_{-I}^{} \cap \spn(\trouble(I))=\{0\}$, i.e. the set~\eqref{eq:equiv:higherorder3} is linearly independent.
%This completes the proof.
\end{proof}

\begin{cor}[$s=0$ case of Theorem~\ref{thm:intro:intersection}]\label{cor:generic_cert}
Let $\V$ be an $\field$-vector space of dimension $n$, let $\X \subseteq \V$ be a conic variety cut out by $p= \delta \binom{n+d-1}{d}$ linearly independent homogeneous degree-$d$ polynomials $f_1,\dots, f_p \in \field[x_1,\dots, x_n]_d$ for a constant $\delta \in (0,1)$, and let $\Phi_{\X}^d: \V^{\otimes d} \rightarrow \field^p$ be the map defined in~\eqref{eq:phi}. 
%There exists a constant $c_d>0$ (that only depends on $d$) such that 
Then a generically chosen linear subspace $\U \subseteq \V$ of dimension
\begin{equation}\label{eq:R}
R \le \frac{p}{ (d-1)! \cdot \binom{n+d-2}{d-1}} = \frac{\delta}{d! } \cdot (n+d-1) % ~~~~(\text{which holds when } R \leq \frac{1}{d! } \cdot \delta (n+d-1))
% R \le \frac{p}{d n^{d-1}} ~~~~(\text{which holds when } R \leq \frac{1}{d! \cdot d} \cdot \delta n)
\end{equation}
% Then a generic linear subspace $\U \subseteq \V$ of dimension
% \ba
% R \leq \delta \Big(\frac{n+d-1}{d}\Big)
% \ea
trivially intersects $\X$ , and is certified as such by our algorithm.
\end{cor}
\begin{proof}
Since $\{f_1,\dots, f_p\}$ is linearly independent, we have that $\rank(\Phi_{\X}^d)=p$. By Theorem~\ref{thm:generic_cert:new}, for a generically chosen tuple of vectors $(u_1,\dots, u_{R}) \in \V^{\times R}$, it holds that
\begin{equation}
%\{\psi_1, \dots, \psi_D\} \cup
\Big\{\Phi_{\X}^d(u_{a_1} \otimes \dots \otimes u_{a_d}) : a \in [R]^{\vee d} \Big\}
\end{equation}
is linearly independent. It follows that $\U:=\spn\{u_1,\dots, u_{R}\}$ trivially intersects $\X$, and is certified as such by our algorithm. %The condition $R \le \delta n/ (d! \cdot d)$ implies $R \le p/ (d n^{d-1})$ since $\binom{n+d-1}{d}/ n^{d-1} \ge n /d!$. 
The two conditions on $R$ are the same since ${\binom{n+d-1}{d}/\binom{n+d-2}{d-1} = (n+d-1)/d}$. 
This completes the proof. 
\end{proof}

%In general, over $\complex$ the maximum dimension of a linear subspace $\U$ trivially intersecting $\X$ is $n-\dim(\X)$, where $\dim(\X)$ denotes the Krull dimension of $\X$~\cite{harris2013algebraic}. We therefore obtain the following consequence of Corollary~\ref{cor:generic_cert}:
%\begin{cor}\label{cor:krulldim}
%Let $\V$ be a $\complex$-vector space of dimension $n$, and let $\X \subseteq \V$ be a conic variety that is cut out by $p = \delta \binom{n+d-1}{d}$ linearly independent homogeneous degree-$d$ polynomials, for a constant $\delta \in (0,1)$. Then
%\ba
%\dim(\X) \leq n- \frac{p}{(d-1)! \binom{n+d-2}{d-1}} = n- \frac{\delta}{d! } \cdot (n+d-1).
%\ea
%%for some constant $c_d>0$ that only depends on $d$. 
%\end{cor}
%Intuitively, this result makes sense: The more equations needed to cut out $\X$, the smaller its dimension should be. The \textit{Hilbert function} of a conic variety $\X$ is the function $h_X: \natural\rightarrow \natural$ that sends $d \in \natural$ to $\binom{n+d-1}{d}-p_d$, where $p_d$ is the largest integer for which $\X$ is contained in a variety cut out by $p_d$ linearly independent homogeneous degree-$d$ polynomials. By the above corollary, we have proven that $\dim(\X) \leq n-\frac{n+d-1}{d!}\left(1-\frac{h_X(d)}{\binom{n+d-1}{d}}\right)$.



==> newproof1.tex <==
%---------------------------------------------------------------------------------------------------%
\section{Algorithm guarantee for generically chosen linear subspaces non-trivially intersecting $\X$}\label{sec:find}
%---------------------------------------------------------------------------------------------------%

In this section, we prove the $s>0$ case of Theorem~\ref{thm:intro:intersection}, which informally says that if $\X$ is non-degenerate of order $d-1$, then for a generically chosen linear subspace $\U\subseteq \V$ of small enough dimension $R:=\dim(\U)$ containing $1 \leq s \leq R$ generically chosen elements of $\X$ (up to scale), then these are the only elements of $\X$ and our algorithm recovers them. We will require the following observation.

\begin{obs}\label{obs:find_sufficient}
Let $d \geq 2$ be an integer, let $s\in [R]$ be an integer, let $v_1,\dots, v_s \in \X$ and $v_{s+1},\dots, v_{R} \in \V$ be vectors, and let $\U = \spn\{v_1,\dots, v_{R}\}$. If the set
\ba\label{eq:linin3}
%\{\psi_1, \dots, \psi_D\} \cup
\Big\{\Phi_{\X}^d(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d}\setminus \Delta_s \Big\}
\ea
is linearly independent, where $\Delta_s = \{(i,\dots,i): i \in [s]\}$, then $\{v_1,\dots, v_{R}\}$ is linearly independent and the only elements of $\U\cap \X$ are $v_1,\dots, v_s$ (up to scale). Furthermore, on input any basis $\{u_1,\dots, u_{R}\}$ of $\U$, Algorithm 1 outputs some non-zero scalar multiples of $v_1,\dots, v_s$ and certifies that these are the only elements of $\U \cap \X$ (up to scale).
\end{obs}

\begin{proof}
By Observation~\ref{obs:find} and Fact~\ref{fact:algorithm_correct}, it suffices to prove that the set of $\alpha \in S^d(\field^{R})$ for which it holds that
\ba\label{eq:lindep}
\sum_{a \in [R]^{\times d}}  \alpha_a \Phi_{\X}^d(u_{a_1}\otimes \dots \otimes u_{a_d})=0
\ea
is equal to $\spn\{Q_i^{\otimes d} : i \in [s]\}$, where $Q=(Q_1,\dots, Q_{R}) \in \GL(\field^{R})$ is the unique invertible linear map for which $(v_1,\dots, v_{R})=(u_1,\dots, u_{R}) Q$. Dualizing, this is equivalent to $S^d(\U) \cap I_d^{\perp}=\spn\{v_1^{\otimes d},\dots, v_s^{\otimes d}\}$, which is in turn equivalent to linear independence of the set~\eqref{eq:linin3}.
%
%
%
%
%
% For any $i \in [s]$, it holds that
%\ba
%\sum_{a \in [R]^{\times d}} (Q_i^{\otimes d})_a \Phi_{\X}^d(u_{a_1}\otimes \dots \otimes u_{a_d})=\Phi_{\X}^d(v_i^{\otimes d})=0,
%\ea
%so clearly $\spn\{Q_i^{\otimes d} : i \in [s]\}$ is contained in the set of $\alpha$ satisfying~\eqref{eq:lindep}. Conversely, if $\alpha$ satisfies~\eqref{eq:lindep}, then
%\ba\label{eq:obs_technical}
%0&=\sum_{a \in [R]^{\times d}}  \alpha_a \Phi_{\X}^d(u_{a_1}\otimes \dots \otimes u_{a_d})\\
%&=\sum_{a \in [R]^{\times d}} \sum_{b \in [R]^{\times d}}  \alpha_a P_{a_1,b_1}\cdots P_{a_d,b_d} \Phi_{\X}^d(v_{b_1}\otimes \dots \otimes v_{b_d})\\
%&=\sum_{b \in [R]^{\vee d}\setminus \Delta_s} \sum_{a \in [R]^{\times d}} \sum_{\sigma \in \mathfrak{S}_d} \alpha_a P_{a_1,b_{\sigma(1)}}\cdots P_{a_d,b_{\sigma(d)}} \Phi_{\X}^d(v_{b_1}\otimes \dots \otimes v_{b_d}),
%\ea
%where $P=Q^{-\t}$. Since~\eqref{eq:linin3} is linearly independent, it follows that each term in the last line indexed by $b \in [R]^{\vee d} \setminus \Delta_s$ is zero. Hence, for all $b \in [R]^{\vee d} \setminus \Delta_s$ it holds that
%\begin{align}
%[(Q^{-1} \otimes \dots \otimes Q^{-1}) \alpha ]_b&=\frac{1}{d!}\sum_{\sigma \in \mathfrak{S}_d}[(Q^{-1} \otimes \dots \otimes Q^{-1}) \alpha ]_{\sigma(b)} \\
%							&=\frac{1}{d!}\sum_{a \in [R]^{\times d}} \sum_{\sigma \in \mathfrak{S}_{d}} P_{a_{1},b_{\sigma(1)}} \cdots P_{a_{d},b_{\sigma(d)}} \alpha_a\\
%							&=0,
%\end{align}
%where the first line follows from permutation invariance, the second line is by definition, and the third line we have verified above. It follows that $\alpha \in \spn \{Q_i^{\otimes d} : i \in [s]\}$. This completes the proof.
\end{proof}




As a consequence of Observation~\ref{obs:find_sufficient}, to show that our algorithm recovers the elements of $\U\cap \X$ for a generically chosen linear subspace $\U \subseteq \V$ containing $s \leq R$ generically chosen elements of $\X$, it suffices to prove that for a generically chosen collection of vectors $v_1,\dots, v_s \in \X, v_{s+1},\dots, v_{R} \in \V$, the set~\eqref{eq:linin3} is linearly independent. This will be established by the following theorem.

\begin{theorem}\label{thm:generic_find:new}
Let $\V$ be an $\field$-vector space of dimension $n$, let $p,R \in \natural$ be positive integers, let $d\geq 2$ be an integer, let $s \in [R]$ be an integer, and let
\ba
\Phi: \V^{\otimes d} \to \field^p
\ea
be a linear map that is invariant under permutations of the $d$ subsystems (i.e. $\Phi \circ P^{\vee}_{\V,d}=\Phi$).
Let $\X_1,\dots, \X_{R} \subseteq \V$ be conic varieties such that $\X_1,\dots, \X_s$ are non-degenerate of order $d-1$, and $\X_{s+1},\dots, \X_{R}$ are non-degenerate of order $d$. If
\begin{equation}
    \rank(\Phi) \geq R (d-1)! \binom{n+d-2}{d-1},
%    D+ R \cdot \binom{N+d-2}{d-1}  < \binom{N+d-1}{d},
\end{equation}
then for a generic choice of $v_1\in \X_1,\dots, v_{R} \in \X_{R}$, the set
\begin{equation} \label{eq:setofvectors1newnew}
%\{\psi_1, \dots, \psi_D\} \cup
\Big\{\Phi(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d} \setminus \Delta_{s}  \Big\}
\end{equation}
is linearly independent , where $\Delta_s=\{(i,\dots,i) : i \in [s]\} \subseteq [R]^{\vee d}.$
\end{theorem}

% \begin{theorem}\label{thm:generic_cert}
% Let $\V$ be an $\field$-vector space of dimension $n$, and for positive integers $d,p$ let
% \ba
% \Phi: \V^{\otimes d} \to \field^p
% \ea
% be a linear map.
% Let $\X_1,\dots, \X_{R} \subseteq \V$ be conic varieties that are non-degenerate of order $d$. If
% \begin{equation}
%     \rank(\Phi) \geq R \cdot d n^{d-1},
% %    D+ R \cdot \binom{N+d-2}{d-1}  < \binom{N+d-1}{d},
% \end{equation}
% then for a generic choice of $v_1 \in \X_1, \dots, v_{R} \in \X_{R}$ it holds  that
% \begin{equation} \label{eq:setofvectors2}
% %\{\psi_1, \dots, \psi_D\} \cup
% \Big\{\Phi(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d} \Big\}
% \end{equation}
% is linearly independent.
% \end{theorem}

First note that, by Fact~\ref{fact:real_vs_complex} and a similar argument as the previous section, it suffices to take ${\field=\complex}$. To show that the set of vectors in~\eqref{eq:setofvectors1newnew} is linearly independent, we consider the total ordering of these vectors given by the relation in Definition~\ref{def:ordering}. % and prove that for every $\Phi(v_{i_1} \otimes \dots \otimes v_{i_d})$ is linearly independent $\{\Phi(v_{a_1} \otimes \dots \otimes v_{a_d}): \}$. 
The proof of Theorem~\ref{thm:generic_find:new} is immediate from the following proposition. 

\begin{prop}\label{prop:newproof1}
If $\field=\complex$, then under the assumptions of Theorem~\ref{thm:generic_find:new}, for generic $v_1 \in \X_1,\dots, v_R \in \X_R$ it holds that
\ba\label{eq:prop:newproof1}
\Phi(v_{i_1} \otimes \dots \otimes v_{i_d}) \notin \spn\Big\{ \Phi(v_{a_1} \otimes \dots \otimes v_{a_d}): (i_1, \dots, i_d) \succ (a_1, \dots, a_d) \in [R]^{\vee d}\setminus \Delta_s \Big\}
\ea
for all $(i_1, \dots, i_d) \in [R]^{\vee d}\setminus \Delta_s$.
\end{prop}
\begin{proof}

The proof is very similar to that of Proposition~\ref{prop:newproof}, and also uses Proposition~\ref{prop:newproof} (note that this statement is nearly identical, except for the fact that here $\X_1,\dots,\X_s$ are allowed to be non-degenerate of order $d-1$, instead of $d$, and correspondingly in~\eqref{eq:prop:newproof1} we do not consider the vectors $v_{i}^{\otimes d}$ with $i \in [s]$). For each $i \in [R]$, let $\X_{i,1},\dots, \X_{i,q_{i}}$ be the irreducible components of $\X_i$. Then the irreducible components of $\X_1 \times \dots \times \X_{R}$ are $\X_{1,j_1} \times \dots \times \X_{R,j_{R}}$ as $j_1,\dots, j_{R}$ range over $[q_1],\dots, [q_{R}]$, respectively. It suffices to prove that~\eqref{eq:prop:newproof1} holds on a Zariski open dense subset of each component. To ease notation, we redefine $\X_1=\X_{1,j_1}$, \dots, $\X_R=\X_{R,j_R}$, and prove that $~\eqref{eq:prop:newproof1}$ holds on a Zariski open dense subset of $\X_1 \times \dots \times \X_{R}$.

For each $I=(i_1,\dots,i_d)\in [R]^{\vee d}\setminus \Delta_s$, let
\ba
\trouble(I)=\Big\{ a \in [R]^{\vee d}~:~ \{a_1, \dots, a_d \} = \{i_1,\dots, i_d\} \text{ and } (i_1, \dots, i_d) \succ (a_1, \dots, a_d) \in [R]^{\vee d} \setminus \Delta_s\Big\},
\ea
where $\succ$ is defined in Definition~\ref{def:ordering}.
%Finally, let $G=G_1\cup \dots \cup G_d$. Note that the set~\eqref{eq:setofvectors1} is linearly independent if and only if $G$ is linearly independent and $\left[\ker(\Phi)\cap S^d(\V)\right] \cap \spn\{G\}=\{0\}$. In turn, this is equivalent to the statement that for all $k \in [d]$ and $I=(i_1,\dots, i_d)\in [R]^{\vee d}$ with $\abs{I}=k$, it holds that $T(I)$ is linearly independent and
%\ba\label{eq:lininequiv}
%T(I) \cap \left[ \left[\ker(\Phi)\cap S^d(\V)\right] + \spn\left\{\bigcup_{k' \in [k-1]} G_{k'} \setminus T(I)\right\}\right]=\{0\}.
%\ea
%$\trouble(I)$ corresponds to all those terms where the indic
Here $\{a_1, \dots, a_d\}=\{i_1, \dots, i_d\}$ means the distinct indices involved in the term corresponding to $a_1, \dots, a_d$ are exactly the distinct indices among $i_1, \dots, i_d$ (note that some may be repeated). Note that this $T(I)$ is the same as the $T(I)$ defined in the previous section (i.e. it automatically holds that $(a_1,\dots, a_d) \notin \Delta_s$ for all $a \in T(I)$ by how we have chosen the ordering $\succ$; this in fact did not need to be imposed in the above definition).

%Finally, let $G_{d+1}$ be a basis of $\ker(\Phi)\cap S^d(\V)$, and let $G=G_1 \cup \dots \cup G_d \cup G_{d+1}$. Note that the set~\eqref{eq:setofvectors1} is linearly independent if and only if $G$ is linearly independent.
Let $w_1 \vee \dots \vee w_d = P^{\vee}_{\V,d} (w_1 \otimes \dots \otimes w_d)$ when $d$ is a positive integer and $w_1,\dots, w_d \in \V$. Since $\Phi$ is invariant under permutations of the $d$ subsystems, it holds that $\Phi(w_1 \otimes \dots \otimes w_d)=\Phi(w_1 \vee \dots \vee w_d)$ for all $w_1,\dots, w_d \in \V$. The proposition is equivalent to the following claim:

\begin{claim} Suppose $I \in [R]^{\vee d}\setminus \Delta_s$. Then
\begin{align}
\Pi^{\perp}_{\prec I} \big(v_{i_1} \vee \dots \vee v_{i_d}\big) \notin \spn\{ \Pi^{\perp}_{\prec I} (v_{a_1}\vee \dots \vee v_{a_d}) : a \in \trouble(I) \}\label{eq:claim:higherorder2:new}  %\\
%\Pi^{\perp}_{<I}  \text{ is the projector perpendicular to }  &\text{span}\big(\big \cup_{k' \le k} G_{k'} \setminus \trouble(I)  \big)
%P^{\vee}_{\V,d}\Big(v_{i_1} \otimes v_{i_2} \otimes \dots \otimes v_{i_d}\Big) \notin \text{span}\Big(\Big\{ P^{\vee}_{\V,d}(v_{a_1} \otimes \dots \otimes v_{a_d}) ~:~ |\{ a_1, \dots, a_d\}| \le |\{i_1, \dots, i_d\}| \Big\}\Big),
\end{align}
 for generically chosen $v_1\in \X_1,\dots, v_{R} \in \X_{R}$, where $\Pi_{\prec I}^{\perp}$ is the orthogonal projection onto the subspace of $S^d(\V)$ orthogonal to
 \ba\label{eq:im_pi_I}
\Z_I:=\ker(\Phi)\cap S^d(\V) + \spn\{v_{a_1} \vee \dots \vee v_{a_d}: a \in [R]^{\vee d}\setminus (\trouble(I)\cup \Delta_s) \quad \text{and} \quad (i_1, \dots, i_d) \succ (a_1, \dots, a_d)\}.
 \ea
\end{claim}
%To see why the claim implies the proposition, note that
%\ba
%\ker(\Phi)\cap S^d(\V) + \{v_{a_1} \vee \dots \vee v_{a_d}: (i_1, \dots, i_d) \succ (a_1, \dots, a_d) \in [R]^{\vee d} \} \subseteq \ker(\Pi_{\prec I}^{\perp}) \cup P^{\vee}_{\V,d}
%\ea
To see why the claim is equivalent, note that~\eqref{eq:prop:newproof1} holds if and only if
\ba
v_{i_1} \vee \dots \vee v_{i_d} \notin \spn\{v_{a_1}\vee \dots \vee v_{a_d} : (i_1,\dots, i_d) \succ (a_1,\dots, a_d) \in [R]^{\vee d}\setminus \Delta_s\} + \ker(\Phi)\cap S^d(\V),
\ea
and~\eqref{eq:im_pi_I} holds if and only if
\ba
v_{i_1} \vee \dots \vee v_{i_d} \notin \spn\{v_{a_1}\vee & \dots \vee v_{a_d} : a \in T(I)\} + \Z_I,
\ea
but the righthand sides of these expressions are equal.

%we can order all the vectors in $G$ in any order with the vectors in $G_{d+1}$ first, followed by those in $G_d$, and so on, until $G_1$. The above claim implies that each vector in this sequence is not contained in the span of the vectors before it, so $G$ is linearly independent. \\
%Indeed, suppose that
%Indeed, suppose that $\left[\ker(\Phi)\cap S^d(\V)\right] \cap \spn\{G\}=\{0\}$. For each $k \in [d]$ fix any ordering of the set of tuples $I=(i_1,\dots, i_d)\in [R]^{\vee d}$ for which $\abs{I}=k$, choose the minimal $k\in [d]$, for which there exists $I \in [R]^{\vee d}$ for which~\eqref{eq:lininequiv} does not hold. Then there exists $u \in \trouble(I), v \in \ker(\Phi)\cap S^d(\V), w\in \spn\left\{\bigcup_{k' \in [k-1]} G_{k'} \setminus \trouble(I)\right\}$ for which $u=v+w$.
%\begin{claim}
%\textit{For all $k \in [d]$ and $I=(i_1,\dots, i_d)\in [R]^{\vee d}$ with $\abs{I}=k$, for generic $v_1,\dots, v_{R} \in \V$ it holds that $\trouble(I)$ is linearly independent and
%\ba
%\trouble(I) \cap \left[ \left[\ker(\Phi)\cap S^d(\V)\right] + \spn\left\{\bigcup_{k' \in [k-1]} G_{k'} \setminus \trouble(I)\right\}\right]=\{0\}.
%\ea}
%\end{claim}
%Indeed, if $G$ is linearly independent and $\left[\ker(\Phi)\cap S^d(\V)\right] \cap \spn\{G\}=\{0\}$, then it is clearly the case that
To complete the proof, we prove the claim. For each choice of vectors $v_1\in \X_1,\dots, v_R \in \X_R$, and each $a \in [R]$, $d \in \mathbb{N}$, let
\ba
\U_a^{(d)}=P_{\V,d}^{\vee}(\spn\{v_a\} \otimes \V^{\otimes d-1}).
\ea
For each $I=(i_1,\dots, i_d)\in [R]^{\vee d}\setminus \Delta_s$, let
\ba
\U_{-I}=\ker(\Phi)\cap S^d(\V) + \spn\bigg\{\bigcup_{a \in [R]\setminus \{i_1,\dots, i_d\}} \U_a^{(d)} \bigg\}.
\ea
Then $\dim(\U_a^{(d)}) \leq \binom{n+d-2}{d-1}$ and
% \ba
% \U_a \coloneqq \spn\{v_a\} \otimes \V^{\otimes d-1}+\V \otimes \spn\{v_a\} \otimes \V^{\otimes d-2} +\dots + \V^{\otimes d-1} \otimes \spn\{v_a\}.
% \ea
% For each $I=(i_1,\dots, i_d)\in [R]^{\vee d}$, let
% \ba
% \U_{-I}=\spn\bigg\{G_0 \cup \bigcup_{a \in [R]\setminus \{i_1,\dots, i_d\}} \U_a\bigg\}.
% \ea
% Then $\dim(\U_a)\le d n^{d-1}$, and %\binom{n+d-2}{d-1}$, and
\ba
\dim(\U_{-I})&\leq \dim(\ker(\Phi)\cap S^d(\V))+(R-k) \binom{n+d-2}{d-1} \\
			&=\binom{n+d-1}{d}-\rank(\Phi)+(R-k) \binom{n+d-2}{d-1} \\
			&\le \binom{n+d-1}{d} - k (d-1)! \binom{n+d-2}{d-1} \quad (\text{from }\eqref{eq:ranklb}, \text{ and } (d-1)!\ge 1),
%			&\leq n^d - k d n^{d-1}. %\binom{N+d-1}{d}-k\binom{N+d-2}{d-1}.
\ea
where $k:=|\{i_1,\dots,i_d\}|$.

Let $\tilde{\Pi}^{\perp}_{-I}$ be the orthogonal projection onto $\U_{-I}^{\perp}$, the orthogonal complement of $\U_{-I}$ in $S^d(\V)$.
We make three observations: % about $\U_{-I}$:
\begin{itemize}
    \item[(i)]  $\U_{-I}$ only depends on $\{v_j : j \notin \{i_1, \dots, i_d\}\}$, and is independent of  $v_{i_1}, \dots, v_{i_d}$.
\item[(ii)] $\U_{-I} \supseteq \Z_I$.%Hence $\text{range}(\Pi^\perp_{-I}) \subseteq \text{range}(\Pi^{\perp}_{<I})$.
\item[(iii)] $\text{rank}(\tilde{\Pi}^\perp_{-I}) = \binom{n+d-1}{d} - \dim(\U_{-I}) \ge k (d-1)! \binom{n+d-2}{d-1}$.
%$\rank(\Phi)-(R-k) \binom{n+d-2}{d-1} \ge k \binom{n+d-2}{d-1}$. %$\ge \rank(\Phi)-(R-k)d n^{d-1}\geq k \cdot d n^{d-1}.$
\end{itemize}
By observation (ii), to establish the claim it suffices to prove that for generically chosen $v_1\in \X_1,\dots, v_{R} \in \X_{R}$, it holds that
\begin{align} \label{eq:equiv:higherorder3}
   \tilde{\Pi}^{\perp}_{-I} \big(v_{i_1} \vee \dots \vee v_{i_d}\big) \notin \spn\{ \tilde{\Pi}^{\perp}_{-I} (v_{a_1}\vee \dots \vee v_{a_d}) : (a_1,\dots, a_d) \in \trouble(I) \}.
\end{align}
Since the subset of $\X_1\times \dots \times \X_{R}$ satisfying~\eqref{eq:equiv:higherorder3} is constructible, and a constructible set contains an open dense subset of its closure, it suffices to prove that this subset is Zariski dense.
%Let $\U_{-I}^{\perp} \subseteq S^d(\V)$ be the orthogonal complement to $\U_{-I}$ in $S^d(\V)$. Then $\dim(\U_{-I}^{\perp})=\rank(\tilde{\Pi}_{-I}^{\perp})$.
%
%
%
%
%
%\begin{align}
%\U_{-I} \cap \text{span}(\trouble(I)) &= \U_{-I} \cap \text{span}\Big\{(P^{\vee}_{\V,d}(v_{a_1} \otimes \dots \otimes v_{a_d})  : \{a_1, \dots, a_d \} = \{i_1, \dots , i_d\} \Big\} = \{0\}.
%\end{align}

Let $\ell$ denote the largest integer in $[d]$ such that $i_{\ell} = i_1$. From the definition of $\trouble(I)$, for every $(a_1,\dots, a_d) \in \trouble(I)$, we have $a_1 = a_2 = \dots = a_\ell = i_1$ (but $a_{\ell+1}$ may or may not be equal to $i_1$). If $\ell=d$, then $\trouble(I)$ is empty, and $(i_1,\dots, i_d)=(i_1,\dots, i_1)$ with $i_1 > s$. Since $\X_{i_1}$ is non-degenerate of order $d$, it holds that $\spn\{v^{\otimes d} : v \in \X_{i_1}\}=S^d(\V)$. For any choice of $\{v_j: j \neq i\}$, it holds that $\rank(\tilde{\Pi}^{\perp}_{-I}) >0$, so a generic choice of $v_{i_1} \in \X_{i_1}$ satisfies~\eqref{eq:equiv:higherorder3}. By a similar argument as in the proof of Proposition~\ref{prop:newproof}, the claim follows. This completes the proof in the case $\ell=d$.

%In more details, we have demonstrated the existence of a set
%\ba\label{eq:zariski_dense}
%\bigcup_{(v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d)} (v_1,\dots,v_{i_1-1}) \times \A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \times (v_{i_1+1}, \dots, v_{d})
%\ea
%such that~\eqref{eq:equiv:higherorder3} holds for every element, where $\A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \subseteq \X_{i_1}$ is a Zariski open dense for every choice of $(v_1,\dots,v_{\hat{i_1}},v_{i_1+1},\dots, v_d)$. The set defined in~\eqref{eq:zariski_dense} is Zariski-dense in $\X_1 \times \dots \times \X_R$. Indeed, any non-empty Zariski open subset $\C \subseteq \X_1 \times \dots \times \X_R$ must intersect some $(v_1,\dots,v_{i_1-1})\times \X_{i_1} \times (v_{i_1+1}, \dots, v_{d})$ non-trivially. It follows that $\C$ must intersect $(v_1,\dots,v_{i_1-1}) \times \A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \times (v_{i_1+1}, \dots, v_{d})$ non-trivially, and hence it must intersect~\eqref{eq:zariski_dense} non-trivially. This completes the proof of this case.

The rest of the proof is essentially identical to that of Proposition~\ref{prop:newproof}, but instead of applying an inductive hypothesis we apply Proposition~\ref{prop:newproof} itself. We henceforth assume $1 \le \ell \le d-1$, and prove the claim by applying Proposition~\ref{prop:newproof} with $(d-\ell)$. 
%Note that $v_{i_1}$ is chosen generically. 
%\anote{ $v_{i_1}$ is chosen generically from the variety}   
For each choice of $v_{i_1} \in \X_{i_1}$, define a linear map
\ba
\tilde{\Phi}:\V^{\otimes (d-\ell)} \to S^d(\V)
\ea
by $\tilde{\Phi}(u)=\tilde{\Pi}^{\perp}_{-I}(v_{i_1}^{\otimes \ell} \otimes u)$. Then
\ba
\W'_{(d-\ell)}:=\setft{Im}(\tilde{\Phi}^*)=v_{i_1}^{\otimes \ell} \hook \U_{-I}^{\perp}
\ea
(recall that $(\cdot)^*$ denotes the conjugate-transpose). For generically chosen $v_{i_1} \in \X_{i_1}$, by Lemma~\ref{lemma:generic_hook:new} it holds that $\W'_{(d-\ell)} \subseteq S^{d-\ell}(\V)$ and
\ba\label{eq:ranklb:2}
\rank(\tilde{\Phi}) = \dim(\W'_{(d-\ell)}) = \dim\big(v_{i_1}^{\otimes \ell} \hook \U_{-I}^{\perp} \big) \geq \frac{1}{\binom{n+\ell-1}{\ell}} \cdot \dim(\U_{-I}^{\perp}) 
%\ge \frac{\rank(\Phi)-(R-k) \binom{n+d-2}{d-1}}{\binom{n+\ell-1}{\ell}} .
\ge k(d-1)!\cdot \frac{  \binom{n+d-2}{d-1}}{\binom{n+\ell-1}{\ell}} .
\ea
Let $\W^{\perp}_{(d-\ell)}$ represent the subspace of $\W'_{(d-\ell)}$ that is orthogonal to $\U^{(d-\ell)}_{i_1}$, and let $\Phi_{(d-\ell)}$ be the orthogonal projection onto the subspace $\W^{\perp}_{(d-\ell)}$. Note by our ordering $\prec$, and our definition of $\trouble(I)$, 
\ba\label{eq:newproof:covered1}
    \Big\{ v_{a_{\ell+1}}\vee \dots \vee v_{a_{d}} : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d)\in \trouble(I) \quad \text{and} \quad  a_{\ell+1} = i_1 \Big\} &\subseteq \U^{(d-\ell)}_{i_1},
\ea
    and
    \ba\label{eq:claim:higherorder2:new}
        \Big\{ v_{a_{\ell+1}}\vee& \dots \vee v_{a_{d}} : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d)\in \trouble(I) \quad \text{and} \quad  a_{\ell+1} \neq i_1 \Big\}\\
        &=\Big\{ v_{a_{\ell+1}} \vee \dots \vee v_{a_{d}} : (a_{\ell+1},\dots, a_d) \in \trouble(i_{\ell+1}, \dots, i_d) \Big\},
        \ea
%    \Big\{ v_{a_1} \otimes \dots \otimes v_{a_{d}}: a\in \trouble(I) \quad \text{and} \quad a_{\ell+1} \ne i_1 \Big\} &= \Big\{ v_{i_1}^{\otimes \ell} \otimes v_{a_{\ell+1}} \otimes \dots \otimes v_{a_{d}} \in \trouble(I) : \{a_{\ell+1},\dots,  a_{d}\} = \{i_{\ell+1}, \dots, i_d\} \Big\}. \label{eq:newproof:covered2}
%\ea
%Moreover for every vector $v_{a_1} \otimes \dots \otimes v_{a_{d}} \in \trouble(I)$ not covered in \eqref{eq:newproof:covered}, we have that $\{a_{\ell+1}, \dots, a_{d} \} = \{i_{\ell+1}, \dots, i_d \}$.  
%Hence Claim A, i.e., \eqref{eq:claim:higherorder2:new}, now follows from the following claim: 
where
   \ba
\trouble(i_{\ell+1}, \dots, i_d)=\Big\{ (a_{\ell+1},\dots, a_d) \in [R]^{\vee (d-\ell)}:& \{a_{\ell+1}, \dots, a_d\}=\{i_{\ell+1}, \dots, i_d\}\\
&\text{and} \; (i_{\ell+1}, \dots, i_d) \succ (a_{\ell+1}, \dots, a_d) \Big\}.
\ea
%}
%Note that $\trouble(i_{\ell+1}, \dots, i_d)$ also contains some extra vectors compared to the ones in \eqref{eq:newproof:covered2} (since it does not impose that $a_1 = i_1, \dots, a_\ell = i_\ell$). \bnote{Does it actually contain extra vectors?}
Note that
\ba
\rank(\Phi_{(d-\ell)}) &= \dim(\W^{\perp}_{(d-\ell)}) \ge \dim(\W'_{(d-\ell)})-\binom{n+d-\ell-2}{d-\ell-1} \\
%&\ge \frac{\rank(\Phi)-(R-k) \binom{n+d-2}{d-1}}{\binom{n+\ell-1}{\ell}} -\binom{n+d-\ell-2}{d-\ell-1} \\
&\ge \frac{k (d-1)! \binom{n+d-2}{d-1} }{\binom{n+\ell-1}{\ell}} -\binom{n+d-\ell-2}{d-\ell-1} \\
&\ge \frac{k (d-1)!}{\binom{d-1}{\ell}} \cdot\binom{n+d-\ell-2}{d-\ell-1} -\binom{n+d-\ell-2}{d-\ell-1}\\
&\ge (k-1) \cdot (d-\ell-1)! \cdot \binom{n+d-\ell-2}{d-\ell-1},
\ea
where the penultimate line follows from $\binom{n+d-2}{d-1} \cdot \binom{d-1}{\ell}\ge \binom{n+d-\ell-2}{d-\ell-1} \cdot \binom{n+\ell-1}{\ell}$.
Furthermore, $\Phi_{(d-\ell)}=\Phi_{(d-\ell)} \circ P^{\vee}_{\V,(d-\ell)}$, $\trouble(i_{\ell+1}, \dots,i_d)\subseteq (i_{\ell+1},\dots, i_d)^{\vee (d-\ell)}$, $\abs{\{i_{\ell+1}, \dots,i_d\}}=k-1$, and the varieties $\X_{i_{\ell+1}},\dots, \X_{i_d}$ are non-degenerate of order $d-\ell$. It follows from Proposition~\ref{prop:newproof} with degree $(d-\ell)$, $R=k-1$, and the operator $\Phi=\Phi_{(d-\ell)}$ that
\begin{align} \label{eq:equiv:higherorder4}
\Phi_{(d-\ell)} \big(v_{i_{\ell+1}} \vee \dots \vee v_{i_d}\big)\notin \spn\{ \Phi_{(d-\ell)}  (v_{a_{\ell+1}}\vee \dots \vee v_{a_{d}}) : (a_{\ell+1},\dots,a_d) \in \trouble(i_{\ell+1},\dots, i_d ) \}
\end{align} 
for generically chosen $v_{i_{\ell+1}}\in \X_{i_{\ell+1}}\dots, v_{i_d} \in \X_{i_{d}}$.
%Moreover the subspace $\W^{\perp}_{d-\ell}$ corresponding to $\Phi_{d-\ell}$ is also a symmetric subspace. Furthermore, $\trouble(i_{\ell+1}, \dots,i_d) \subset (\spn\{v_{i_{\ell+1}},\dots,v_{i_d}\})^{\otimes d-\ell}$ and $|v_{i_{\ell+1}},\dots,v_{i_d}\}|=k-1$. Also $\Phi_{d-\ell}$ is fixed independent of the generic choices of $v_{i_{\ell+1}},\dots,  v_{i_d}$ (note that $\Phi_{d-\ell}$ may depend on $v_{i_1}$), and  no irreducible component of any of the varieties $\X_1,\dots, \X_{R}$ has equations in degree $d-\ell$.
%%\noindent {\em {\bf Claim B.} For generic $v_1 \in \X_1,\dots, v_{R} \in \X_{R}$, we have    
%We now use the inductive hypothesis i.e., Proposition~\ref{prop:newproof} with degree $(d-\ell)$, $R=k-1$, and the operator $\Phi=\Phi_{d-\ell}$ to conclude 
%\begin{align} \label{eq:equiv:higherorder4}
%   &\Phi_{d-\ell} \big(v_{i_{\ell+1}} \otimes \dots \otimes v_{i_d}\big) \text{ is linearly independent of } \{ \Phi_{d-\ell}  u : u \in \trouble(i_{\ell+1},\dots, i_d ) \}.
%\end{align} 

This establishes~\eqref{eq:equiv:higherorder3} as follows: First, note that~\eqref{eq:equiv:higherorder3} is equivalent to
\begin{align}
   \tilde{\Pi}^{\perp}_{-I} \big(v_{i_1}^{\otimes \ell} \otimes (v_{i_{\ell+1}}\vee \dots \vee v_{i_d})\big) \notin \spn\{ \tilde{\Pi}^{\perp}_{-I} \big((v_{i_1})^{\otimes \ell} \otimes (v_{a_{\ell+1}} \vee \dots \vee v_{a_d})\big) : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d) \in \trouble(I) \}.
\end{align}
Indeed, since $\tilde{\Pi}^{\perp}_{-I}=\tilde{\Pi}^{\perp}_{-I} \circ P^{\vee}_{\V,d}$, it also holds that $\tilde{\Pi}^{\perp}_{-I}=\tilde{\Pi}^{\perp}_{-I} \circ (\mathbb{1}_{\V}^{\otimes \ell} \otimes P^{\vee}_{\V,(d-\ell)})$. By the definition of $\tilde{\Phi}$, this is equivalent to
\begin{align}
   \tilde{\Phi}(v_{i_{\ell+1}}\vee \dots \vee v_{i_d}) \notin \spn\{ \tilde{\Phi}(v_{a_{\ell+1}} \vee \dots \vee v_{a_d}) : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d) \in \trouble(I) \},
\end{align}
i.e.
\begin{align}
v_{i_{\ell+1}}\vee \dots \vee v_{i_d} \notin \spn\{ v_{a_{\ell+1}} \vee \dots \vee v_{a_d} : (i_1,\dots, i_1,a_{\ell+1},\dots, a_d) \in \trouble(I) \} + \ker(\tilde{\Phi}) \cap S^{d-\ell}(\V),\nonumber\\
\label{eq:right1}
\end{align}
where $\ker(\tilde{\Phi}) \cap S^{d-\ell}(\V)=\im((\tilde{\Phi})^*)^{\perp}\cap S^{d-\ell}(\V)=(W'_{(d-\ell)})^{\perp}\cap S^{d-\ell}(\V).$ Similarly,~\eqref{eq:equiv:higherorder4} is equivalent to
\begin{align}\label{eq:right2}
v_{i_{\ell+1}} \vee \dots \vee v_{i_d} \notin \spn\{ v_{a_{\ell+1}}\vee \dots \vee v_{a_{d}} : (a_{\ell+1},\dots,a_d) \in \trouble(i_{\ell+1},\dots, i_d ) \} + \ker(\Phi_{(d-\ell)}),
\end{align}
where $\ker(\Phi_{(d-\ell)})=\U_{i_1}^{(d-\ell)} + (W'_{(d-\ell)})^{\perp}\cap S^{(d-\ell)}(\V).$ By~\eqref{eq:newproof:covered1} and~\eqref{eq:claim:higherorder2:new}, the righthand side of~\eqref{eq:right1} is contained in the righthand side of~\eqref{eq:right2}. By a similar argument as in the end of the proof of Proposition~\ref{prop:newproof}, this shows that~\eqref{eq:equiv:higherorder3} holds on a Zariski open dense subset of $\X_1\times \dots \times \X_R$.
%\ba\label{eq:zariski_dense2}
%\bigcup_{v\in \B} (v_1,\dots,v_{i_1-1}) \times \A_{v_1, \dots, v_{\hat{i_1}},v_{i_1+1},\dots, v_d} \times (v_{i_1+1}, \dots, v_{d})
%\ea
%Thus,~\eqref{eq:equiv:higherorder3} holds for generic choices of $v_1 \in \X_1,\dots, v_R \in \X_R$.
%This now implies Claim A (i.e., \eqref{eq:claim:higherorder2:new}) as follows:  by definition, $\Phi' (u) = \tilde{\Pi}^{\perp}_{-I} (v_{i_1}^{\otimes \ell} \otimes u)$, where $\Phi'$ is the projector onto the subspace $\W'_{d-\ell}$ and  $\Phi_{d-\ell}$ is the projector of the $\W^{\perp}_{d-\ell}$ (the subspace of $\W'_{d-\ell}$ that is orthogonal to $\U^{(d-\ell)}_{i_1}$). Also from \eqref{eq:newproof:covered1} and  \eqref{eq:newproof:covered2}, every $v_{a_1} \otimes \dots \otimes v_{a_{d}} \in \trouble(I)$ is either contained in $\{ v_{i_1}^{\otimes \ell} \otimes \U^{(d-\ell)}_{i_1} \cup v_{i_1}^{\otimes \ell} \otimes \trouble(i_{\ell+1}, \dots, i_{d}) \}$. 
%% Since $\abs{\{i_1,\dots, i_d\}}=k$, and
%% \ba
%% \rank \geq \frac{1}{\binom{n+\ell-1}{\ell}} \dim(\U_{-I}^{\perp}) ,
%% \ea
%% it follows from the induction hypothesis that for a generic choice of $v_{i_1}\in \X_{i_1},\dots, v_{i_d}\in \X_{i_d}$ it holds that $(f \hook_1 \U_{-I}^{})\cap (f \hook_1 \spn(\trouble(I)))=\{0\}$. Since $f\in \V^*$ is also generic, this implies $\U_{-I}^{} \cap \spn(\trouble(I))=\{0\}$, i.e. the set~\eqref{eq:equiv:higherorder3} is linearly independent.
%This completes the proof.
\end{proof}


\begin{cor}[$1\leq s \leq R$ case of Theorem~\ref{thm:intro:intersection}]\label{cor:generic_find}
Let $\X \subseteq \V=\field^n$ be a conic variety cut out by $p= \delta \binom{n+d-1}{d}$ linearly independent homogeneous degree-$d$ polynomials $f_1,\dots, f_p \in \field[x_1,\dots, x_n]_d$ for a constant $\delta \in (0,1)$. Suppose furthermore that $\X$ is non-degenerate of order $d-1$. Then for a linear subspace $\U \subseteq \V$ of dimension
\ba
R \le \frac{1}{d!} \cdot \delta (n+d-1),
\ea
spanned by a generically chosen element of $\X^{\times s} \times \V^{\times R-s}$, $\U$ has only $s$ elements in its intersection with $\X$ (up to scalar multiples), and Algorithm 1 recovers these elements from any basis of $\U$.
\end{cor}
\begin{proof}
Since $\{f_1,\dots, f_p\}$ is linearly independent, it follows that $\rank(\Phi_{\X}^d)=p$, so by Theorem~\ref{thm:generic_find:new}, for a generically chosen tuple of vectors
\ba
(v_1,\dots, v_s, v_{s+1},\dots, v_{R}) \in \X^{\times s} \times \V^{\times {R-s}}
\ea
the set
\begin{equation}
%\{\psi_1, \dots, \psi_D\} \cup
\Big\{\Phi_{\X}^d(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d} \setminus \Delta_{s}  \Big\}
\end{equation}
is linearly independent, where $\Delta_s=\{(i,\dots,i) : i \in [s]\} \subseteq [R]^{\vee d}.$ Let $\U:=\spn\{v_1,\dots, v_{R}\}$. By Observation~\ref{obs:find_sufficient}, it follows that $v_1,\dots, v_s$ are the only elements of $\U \cap \X$ (up to scale), and they are recovered by Algorithm 1. This completes the proof.
\end{proof}




==> scratch.tex <==

\section{SCRATCH}



For a conic variety $\X \subseteq \V$ and a linear subspace $\U \subseteq \V$, we define the \textit{simultaneous $\X$-rank} of $\U$ to be the smallest integer $r$ for which there exists $v_1,\dots, v_r \in \X$ such that $\U \subseteq \spn\{v_1,\dots, v_r\}$.





Let $n$ and $m$ be positive integers, let $\V$ and $\W$ be $\field$-vector spaces of dimensions $n$ and $\tilde{n}$ respectively, let $\{y_1,\dots, y_{\tilde{n}}\} \subseteq \W^*$ be a basis for $\W^*$, let $T \in \V \otimes \W$ be a tensor, and let $T(\W^*) \subseteq \V$ be the image of $T: \W^* \rightarrow \V$. Finally, let $\X \subseteq \V$ be a non-degenerate conic variety. Then the following numbers are equal:
\begin{enumerate}
\item The smallest integer $r$ for which there exists $v_1,\dots, v_r \in \X$ such that $T(\W^*)\subseteq \spn\{v_1,\dots,v_r\}$.
\item The smallest integer $r$ for which there exists $v_1,\dots, v_r \in \X$ such that $T(y_i)\in \spn\{v_1,\dots,v_r\}$ for all $i \in [{\tilde{n}}]$.
\item The smallest integer $r$ for which there exists $v_1,\dots, v_r \in \X$ and $w_1,\dots, w_r \in \W$ such that $T=\sum_{a\in [R]} v_a \otimes w_a$.
\end{enumerate}
Indeed, equality of the first two numbers is obvious, and equality of the first and third numbers follows from the fact that $T(\W^*) \subseteq \spn\{v_1,\dots,v_r\}$ if and only if there exists $w_1,\dots, w_r \in \W$ for which $T=\sum_{a\in[R]} v_a \otimes w_a$. We define this number $r$ to be the \textit{simultaneous $\X$-rank} of $T$, and we refer to the set $\{v_1,\dots, v_r\} \subseteq \X$ as a \textit{simultaneous $\X$-rank decomposition} of $T$. If $T(\W^*)\subseteq \spn\{v_1,\dots, v_r\}$ and  $v_1,\dots, v_r\in \X$, but $r$ is not necessarily the simultaneous $\X$-rank of $T$, then we refer to $\{v_1,\dots, v_r\}$ as simply a \textit{simultaneous $\X$ decomposition} of $T$. We say that $\{v_1,\dots, v_r\} \subseteq \X$ is the \textit{unique simultaneous $\X$-rank decomposition} of $T$ if it is a simultaneous $\X$-rank decomposition of $T$ and for any other simultaneous $\X$-rank decomposition $\{u_1,\dots, u_r\} \subseteq \X$ of $T$, there exists a permutation $\sigma \in \mathfrak{S}_r$ for which $v_a \in \spn\{u_{\sigma(a)}\}$ for all $a \in [r]$.

For an $\field$-vector space $\U$ and a non-degenerate, conic variety $\Y \subseteq \U$, the \textit{$\Y$-rank} of a vector $v \in \U$ is the smallest integer $r$ for which there exist $u_1,\dots, u_r \in \Y$ such that
\ba
v=\sum_{a \in [r]} u_a.
\ea
We refer to the set $\{u_1,\dots, u_r\}$ as a $\Y$\textit{-rank decomposition} of $v$. We say that $\{u_1,\dots, u_r\}$ is the \textit{unique $\Y$-rank decomposition} of $v$ if it is the only $\Y$-rank decomposition of $v$. By the above discussion, the simultaneous $\X$-rank of a tensor $T \in \V \otimes \W$ is precisely the $S(\X \times \W)$-rank of $T$, where
\ba
S(\X \times \W):=\{v \otimes w : v \in \X \quad \text{and} \quad w \in \W\}\subseteq \V \otimes \W.
\ea
The set $S(\X \times \W)$ forms a non-degenerate, conic variety equal to the affine cone over the Segre embedding of $\proj \X \times \proj \W$ in $\proj(\V \otimes \W)$. Furthermore, $\{v_1,\dots, v_r\} \subseteq \X$ is the unique simultaneous $\X$-rank decomposition of $T$ if and only if
\ba
T=\sum_{a \in [r]} v_a \otimes w_a
\ea
is the unique $S(\X \times \W)$-rank decomposition of $T$, where $w_a := T(v_a^*)$, and $v_a^*$ is the dual vector to $v_a$ with respect to any basis $\{v_1,\dots v_n\}$ for $\V$ that extends $\{v_1,\dots, v_r\}$.

For example, for $\field$-vector spaces $\V_1,\V_2, \V_3$ of dimensions $n_1,n_2,n_3$, the \textit{tensor rank} of a tensor $T \in \V_1 \otimes \V_2 \otimes \V_3$ is defined as the smallest integer $r$ for which
\ba\label{eq:tensor_decomp}
T=\sum_{a \in [r]} v_{a,1} \otimes v_{a,2} \otimes v_{a,3}
\ea
for some $v_{1,1},\dots,v_{r,1}\in \V_1$, $v_{1,2},\dots,v_{r,2}\in \V_2$, $v_{1,3},\dots,v_{r,3}\in \V_3$. This is precisely the simultaneous $\X_1$-rank of $T$, where
\ba
\X_1=\{v_1\otimes v_2 : v_1 \in \V_1, v_2 \in \V_2\}.
\ea

More generally, for a positive integer $r \leq \min\{n_1,n_2\}$, the \textit{$(r,r,1)$-block rank} of $T$ is the smallest integer $r$ for which
\ba
T=\sum_{a \in [r]} v_a \otimes w_a
\ea
for some $v_1,\dots, v_r\in \X_{r}$ and $w_1,\dots, w_r\in \V_3$, where
\ba
\X_r=\{v \in \V_1 \otimes \V_2 : \rank(v: \V_1^*\rightarrow \V_2)\leq r\}.
\ea
This is equal to the simultaneous $\X_r$-rank of $T$.

Our algorithm gives a method of finding a simultaneous $\X$-rank decomposition of a tensor $T$, and verifying that it is unique. In particular, by Corollary~\ref{cor:generic_find} and the above observations, we have the following application of our algorithm to tensor decompositions:

\begin{theorem}\label{thm:generic_find_app}
Let $\X \subseteq \V$ be a conic variety cut out by $p$ linearly independent homogeneous degree-$d$ polynomials, and suppose furthermore that $\X$ has no equations in degree $d-1$. Then for any vector space $\W$, a generic tensor $T \in \V \otimes \W$ of simultaneous $\X$-rank
\ba
r \leq \min\Bigg\{\dim(\W),p \binom{n+d-2}{d-1}^{-1}\Bigg\}
\ea
has a unique simultaneous $\X$-rank decomposition, and our algorithm finds this decomposition.
\end{theorem}
\begin{proof}
Since a generic tensor $T \in \V \otimes \W$ of simultaneous $\X$-rank $r\leq \dim(\W)$ satisfies $\dim(T(\W^*))=r$, there exists $v_1,\dots, v_r \in \X$ for which
\ba
T(\W^*)=\spn\{v_1,\dots, v_r\}.
\ea
Since $T$ is generic and $r \leq p \binom{n+d-2}{d-1}^{-1}$, it follows from Corollary~\ref{cor:generic_find} that $v_1,\dots, v_r$ are the only elements of $\X \cap T(\W^*)$ up to scale, and given any basis $\{u_1,\dots, u_r\}$ for $T(\W^*)$, the vectors $v_1,\dots, v_r$ are recovered (up to scale) by our algorithm. This completes the proof.
\end{proof}

\begin{cor}
A generic tensor in $\field^{n_1}\otimes \field^{n_2} \otimes \field^{n_3}$ of tensor rank
\ba
r \leq \min\Bigg\{n_3, \frac{(n_1-1)(n_2-1)}{4}\Bigg\}
\ea
has a unique tensor rank decomposition, and this decomposition is recovered by our algorithm.
\end{cor}
\begin{proof}
A generic tensor $T\in \field^{n_1}\otimes \field^{n_2} \otimes \field^{n_3}$ of tensor rank $r \leq n_3$, satisfies $\dim(T(\W^*))=r$, so there exists $v_1,\dots, v_r \in \X_1$ for which
\ba
T((\field^{n_1})^*) = \spn\{v_1,\dots, v_r\}.
\ea
Note that $\X_1\subseteq \field^{n_1}\otimes \field^{n_2}$ is non-degenerate and is cut out by $p=\binom{n_1}{2}\binom{n_2}{2}$ linearly independent polynomials of degree $d=2$ (the $2\times 2$ minors). Since $T$ is generic and $r \leq \frac{(n_1-1)(n_2-1)}{4}=p \binom{n+d-2}{d-1}^{-1}$, it follows from Corollary~\ref{cor:generic_find} that $v_1,\dots, v_r$ are the only elements of $\X \cap T((\field^{n_1})^*)$ up to scale, and given any basis $\{u_1,\dots, u_r\}$ for $T((\field^{n_1})^*)$, the vectors $v_1,\dots, v_r$ are recovered (up to scale) by our algorithm. As mentioned above, the unique tensor rank decomposition of $T$ can be easily computed from $v_1,\dots, v_r$. This completes the proof.
\end{proof}

More generally, Theorem~\ref{thm:generic_find_app} can be used to compute $(r,r,1)$-block decompositions as follows:

\begin{cor}
A generic tensor in $\field^{n_1}\otimes \field^{n_2} \otimes \field^{n_3}$ of $(r,r,1)$-block rank
\ba
r \leq \min\Bigg\{n_3, \binom{n_1}{r+1}\binom{n_2}{r+1}\binom{n_1n_2+r-1}{r}^{-1}\Bigg\}
\ea
has a unique $(r,r,1)$-block rank decomposition, and this decomposition is recovered by our algorithm.
\end{cor}
\begin{proof}
This follows from a nearly identical argument to the proof of Corollary~\ref{cor:tensor_decomp}, and the fact that $\X_r \subseteq \field^{n_1}\otimes \field^{n_2}$ is a conic variety cut out by $p=\binom{n_1}{r+1}\binom{n_2}{r+1}$ homogeneous polynomials of degree $d=r+1$, and the fact that $\X_r$ has no equations in degree $r$~\cite{harris2013algebraic}.
\end{proof}

\section{MORE SCRATCH}


Suppose that the unknown set of vectors $\{v_1,\dots, v_s\}$ is linearly independent, and let $\{v_1,\dots, v_{R}\}$ be a basis for $\U$ that extends this set. Let $Q \in \GL(\field^{R})$ be the invertible linear map for which $(v_1,\dots, v_{R})=(u_1,\dots, u_{R})Q$. Then $u_i=\sum_{j=1}^{R} Q^{-1}_{(j,i)} v_j$ for all $i \in [R]$. Substituting this expression into~\eqref{eq:lindep}, we obtain
\ba
0&=\sum_{a \in [R]^{\vee d}} \alpha_a \sum_{b \in [R]^{\vee d}} Q^{-1}_{(b_1,a_1)} \cdots Q^{-1}_{(b_d,a_d)} \Phi_{\X}^d(v_{b_1}\otimes \dots \otimes v_{b_d})\\
&=\sum_{b \in [R]^{\vee d}} \left((Q^{-1})^{\otimes d}\alpha\right)_{b} \Phi_{\X}^d(v_{b_1}\otimes \dots \otimes v_{b_d})\\
&=\sum_{b \in [R]^{\vee d}\setminus \Delta_s} \left((Q^{-1})^{\otimes d}\alpha\right)_{b} \Phi_{\X}^d(v_{b_1}\otimes \dots \otimes v_{b_d}),
\ea
where $\Delta_s = \{(i,\dots,i) : i \in [s]\}$. The notation $(Q^{-1})^{\otimes d}\alpha$ denotes the application of the invertible linear map
\ba
(Q^{-1})^{\otimes d} : S^d(\field^{R}) \rightarrow S^d(\field^{R})
\ea
to the symmetric tensor $\alpha \in S^d(\field^{R})$. The third line follows from the fact that $v_1,\dots, v_s \in \X$, so
\ba
\Phi_{\X}^d(v_1^{\otimes d})=\dots=\Phi_{\X}^d(v_s^{\otimes d})=0.
\ea
Now suppose that the set
\ba\label{eq:linin1}
%\{\psi_1, \dots, \psi_D\} \cup
\Big\{\Phi_{\X}^d(v_{a_1} \otimes \dots \otimes v_{a_d}) : a \in [R]^{\vee d}\setminus \Delta_s \Big\}
\ea
is linearly independent. We now prove two facts:
\begin{enumerate}
\item A symmetric tensor $\alpha \in S^d(\field^{R})$ satisfies~\eqref{eq:lindep} if and only if
\ba
\alpha \in \spn\{Q_i^{\otimes d} : i \in [s]\}.
\ea
\item Whenever Fact~1 holds, $v_1,\dots, v_{s}$ are the only elements of $\X \cap \U$ (aside from scalar multiples).
\end{enumerate}
For Observation~1, by the assumption that~\eqref{eq:linin1} is linearly independent, it follows that $\alpha$ satisfies~\eqref{eq:lindep} if and only if $\left((Q^{-1})^{\otimes d}\alpha\right)_{b}=0$ for all $b \in [R]^{\vee d}\setminus \Delta_s$. Since $(Q^{-1})^{\otimes d}$ is invertible, this is equivalent to
\ba
\alpha \in \spn\{Q_i^{\otimes d} : i \in [s]\}.
\ea
For Observation~2, note that if $v=\sum_{i=1}^{R} \alpha_i v_i \in \X$, then
\ba
0=\Phi_{\X}^d(v^{\otimes d})=\sum_{a \in [l]^{\vee d}} \alpha_{a_1}\cdots \alpha_{a_d} \Phi_{\X}^d(v_{a_1}\otimes \dots \otimes v_{a_d}),
\ea
so by Observation~1, $\alpha_{a_1}\cdots \alpha_{a_d}=0$ for all $a \in [R]^{\vee d} \setminus \Delta_s$. This implies $\alpha_i \neq 0$ for (at most) a single index $i \in [s]$. Thus, $v\in \spn\{v_i\}$.


%
%
%
%Perform Jennrich's algorithm on the tensor
%\begin{align}
%\tilde{R}&=\sum_{a \in [s]} \ket{a} \otimes R_a\\
%\end{align}





\section{Finding planted elements of a variety in a linear subspace}


\begin{lemma}\label{lemma:cardoso_gen}
Let $s \leq l$ be positive integers, let $\V$ be an $\field$-vector space, let $\X \subseteq \V$ be a conic variety cut out by a set of homogeneous degree-$d$ polynomials $f_1,\dots, f_{p}$, let $v_1,\dots, v_l \in \V$ be vectors for which $v_a \in \X$ for all $a \in [s]$, and let $V=(v_1,\dots, v_l) \in \Lin(\field^l, \V)$. Similarly, let $u_1,\dots, u_l \in \V$ be a collection of vectors (not necessarily in $\X$), and let $U=(u_1,\dots, u_l)\in \Lin(\field^l, \V)$. For each $d \in \natural$, let $\Phi_\X^d: \V^{\otimes d} \rightarrow \field^{p}$ be the map defined above. Suppose further that the following two conditions hold:
\begin{enumerate}
\item There exists an invertible matrix $Q \in \GL(\field^l)$ for which $V=UQ.$
\item The set of vectors
\begin{align}
\{\Phi_{\X}^d(v_{a_1} \otimes \dots \otimes v_{a_{d}}) : a \in [l]^{\vee d} \setminus \Delta_s\} \subseteq \field^p
\end{align}
is linearly independent, where $\Delta_s=\{(i,\dots ,i) : i \in [s]\} \subseteq [l]^{\vee d}$.
\end{enumerate}
Then a fully symmetric tensor $T \in S^d(\field^l)$ satisfies
\begin{align}\label{eq:symmetric_zero_combo}
\sum_{a \in [l]^{\vee d}} T_a \Phi_{\X}^d(u_{a_1} \otimes \dots \otimes u_{a_{d}})=0
\end{align}
if and only if
\begin{align}\label{eq:odeco}
T\in \spn\{ Q_{({:,a})}^{\otimes d} : a \in [s]\},
\end{align}
where $Q_{({:,a})}$ denotes the $a$-th column of $Q$. Furthermore, $v_1,\dots, v_s$ are the only elements of $\spn(U)$ contained in $\X$ (up to scale), and these elements can be obtained efficiently from $U$.
\end{lemma}


\begin{proof}
Let $P=(Q^{-1})^\t$. Note that
\begin{align}
\sum_{a \in [l]^{\vee d}} T_a \Phi_{\X}^d&(u_{a_1} \otimes \dots \otimes u_{a_{d}})=\sum_{a \in [l]^{\vee d}} T_a \Phi_{\X}^d( (VQ^{-1})_{(:,a_1)} \otimes \dots \otimes (VQ^{-1})_{(:,a_{d})})\\
						&=\sum_{a \in [l]^{\vee d}} \sum_{b \in [l]^{\vee d}}T_a \sum_{\sigma\in \mathfrak{S}_{d}} \left[P_{(a_1,{b_{\sigma(1)}})} \cdots P_{(a_{d},b_{\sigma(d)})}\right] \Phi_{\X}^d(v_{b_1} \otimes \dots \otimes v_{b_{d}})\\
						&=\sum_{a \in [l]^{\vee d}} \sum_{b \in [l]^{\vee d}\setminus \Delta_s} T_a \sum_{\sigma \in \mathfrak{S}_{d}} \left[P_{(a_{1},b_{\sigma(1)})} \cdots P_{(a_{d},b_{\sigma(d)})}\right] \Phi_\X^d(v_{b_1}\otimes \dots \otimes v_{b_{d}}),
\end{align}
where the first line follows from $V=UQ$, the second follows from the fact that $\Phi_\X^d$ is invariant under permutation of the copies of $\V$, and the third follows from the fact that $v_1,\dots, v_s\in \X$. By Condition 2, this quantity is zero if and only if
\begin{align}\label{eq:pairing_zero}
\sum_{a \in [l]^{\vee d}} T_a \sum_{\sigma \in \mathfrak{S}_d} \left[P_{(a_1,b_{\sigma(1)})} \cdots P_{(a_{d},b_{\sigma(d)})}\right]=0
\end{align}
for all $b \in [l]^{\vee d}\setminus \Delta_s$.

If $T$ satisfies~\eqref{eq:odeco}, then
\begin{align}
\sum_{a \in [l]^{\vee d}} T_a \sum_{\sigma \in \mathfrak{S}_{d}} \left[P_{(a_1,b_{\sigma(1)})} \cdots P_{(a_{d},b_{\sigma(d)})}\right]&=\sum_{\sigma \in \mathfrak{S}_{d}} [(Q^{-1} \otimes \dots \otimes Q^{-1})T]_{(b_{\sigma(1)},\dots, b_{\sigma(d)})}\\
								&=0
\end{align}
for all $b \in [l]^{\vee d}\setminus \Delta_s$, where the first line is algebra and the second line follows from the fact that $[(Q^{-1} \otimes \dots \otimes Q^{-1})T]_b=0$ for all $b \in [l]^{\vee d}\setminus \Delta_s$. Hence, $T$ satisfies~\eqref{eq:symmetric_zero_combo}. Conversely, if $T$ satisfies~\eqref{eq:symmetric_zero_combo}, then
\begin{align}
[(Q^{-1} \otimes \dots \otimes Q^{-1})T]_b&=\sum_{a \in [l]^{\vee d}} P_{( a_1,b_1)} \cdots P_{(a_{d},b_{d})} T_a\\
							&=\frac{1}{d!}\sum_{a \in [l]^{\vee d}} \sum_{\sigma \in \mathfrak{S}_{d}} P_{(a_{\sigma(1)},b_1)} \cdots P_{(a_{\sigma(d)},b_{d})} T_a\\
							&=0
\end{align}
for all $b \in [l]^{\vee d}\setminus \Delta_s$, where the first line is algebra, the second follows from the fact that $T$ is symmetric, and the third follows from~\eqref{eq:pairing_zero}. For each $a \in [s]$, let
\begin{align}
\alpha_a=\left[(Q^{-1} \otimes \dots \otimes Q^{-1})T\right]_{(a,\dots, a)}.
\end{align}
Then
\begin{align}
T= (Q \otimes \dots \otimes Q) (Q^{-1}\otimes \dots \otimes Q^{-1}) T= \sum_{a \in [s]} \alpha_a Q_{(:,a)}^{\otimes d},
\end{align}
so~\eqref{eq:odeco} holds.

We next prove that $v_1,\dots, v_s$ are the only elements of $\spn(U) \cap \X$, up to scale. Let $v= \sum_{a \in [l]} \alpha_a v_a$ be an arbitrary element of $\spn(U)$, where $\alpha_1,\dots, \alpha_l \in \field$. Then
\begin{align}
\Phi_{\X}^d(v^{\otimes d})&=d!\sum_{a \in [l]^{\vee d}} \alpha_{a_1} \cdots \alpha_{a_d} \Phi_{\X}^d(v_{a_1} \otimes \dots \otimes v_{a_d})\\
&=d!\sum_{a \in [l]^{\vee d} \setminus \Delta_s} \alpha_{a_1} \cdots \alpha_{a_d} \Phi_{\X}^d(v_{a_1} \otimes \dots \otimes v_{a_d}).
\end{align}
By Condition 2, this linear combination can only be zero if $\alpha_a =0$ for all $a \in [l]\setminus [s]$ and $\alpha_a\neq 0$ for at most a single index $a \in [s]$, i.e., if $v \in \spn\{v_a\}$ for some $a \in [s]$.

To recover $v_1, \dots, v_s$ efficiently from $U$ (up to scale), note that it suffices to recover $Q_{(:,1)}^{\otimes d},\dots, Q_{(:,s)}^{\otimes d}$ up to scale. Let $\{R_1,\dots, R_s\}$ be a basis for $\spn\{Q_{(:,a)}^{\otimes d}: a \in [s]\}$, which can be efficiently computed by solving the linear equation~\eqref{eq:symmetric_zero_combo}. So there exists an invertible matrix $G \in \GL(\field^s)$ for which $(R_1,\dots, R_s)=(Q_{(:,1)}^{\otimes d},\dots, Q_{(:,s)}^{\otimes d})G$. Consider the tensor
\begin{align}
\tilde{R}&=\sum_{a \in [s]} e_a \otimes R_a\\
	&=\sum_{b \in [s]} G^{\t} e_b \otimes Q_{(:,s)}^{\otimes d},
\end{align}
which is the unique tensor rank decomposition of $\tilde{R}$. To recover $Q_{(:,1)}^{\otimes d},\dots, Q_{(:,s)}^{\otimes d}$ up to scale, this decomposition can be efficiently computed using Jennrich's algorithm. This completes the proof.
\end{proof}


\begin{definition}
For $\field$-vector spaces $\V$ and $\W$, a conic, non-degenerate variety $\X \subseteq \V$, and a tensor $T \in \V \otimes \W$, we define the \textit{$(\X,\W)$-rank} of $T$, denoted $\setft{R}_{(\X,\W)}(T)$, to be the smallest integer $l$ for which there exist $v_1,\dots, v_l \in \X$ and $w_1,\dots, w_l \in \W$ such that $T=\sum_{a \in [l]} v_a \otimes w_a$.
\end{definition}
Note that $\setft{R}_{(\X,\W)}(T)$ is equal to the smallest number $l$ for which there exist $v_1,\dots, v_l \in \X$ that satisfy $T(\W^*) \subseteq \spn \{ v_1,\dots, v_l\}$. Note also that if $\X$ is a Segre variety, then $\setft{R}_{(\X,\W)}(T)=\setft{R}(T)$ is the standard tensor rank.

\begin{theorem}\label{thm:tensor_decomp}
Let $\V$ and $\W$ be $\complex$-vector spaces, let $\X\subseteq \V$ be a conic, non-degenerate and irreducible variety cut out by degree-$d$ homogeneous polynomials, and let $T \in \V \otimes \W$ be a tensor. If $T$ admits an $(\X,\W)$-decomposition of the form $T=\sum_{a \in [l]} v_a \otimes w_a$ for which $\{w_a : a \in [l]\}$ is linearly independent and
\ba\label{eq:linintheorem}
\{\Phi_{\X}^d(v_{a_1}\otimes \dots \otimes v_{a_d}) : a \in [l]^{\vee d} \setminus \Delta_l\}
\ea
is linearly independent, where $\Delta_l=\{(i,\dots, i) : i \in [l]\}$, then the following statements hold:
\begin{enumerate}
\item $\setft{R}_{(\X,\W)}(T)=l$.
\item $T=\sum_{a \in [l]} v_a \otimes w_a$ is the unique $(\X, \W)$-rank decomposition of $T$.
\item The decomposition $T=\sum_{a \in [l]} v_a \otimes w_a$ can be obtained efficiently from $T$.
\end{enumerate}
\end{theorem}
\begin{proof}
Since the set~\eqref{eq:linintheorem} is linearly independent, it follows from Lemma~\ref{lemma:cardoso_gen} that the vectors $v_1,\dots, v_l$ are the unique elements of $T(\W^*)\cap \X$ up to scale, and they can be obtained efficiently from $T$. It also follows that $\{v_1,\dots, v_l\}$ is linearly independent, so there are unique vectors $w_1,\dots, w_l \in \W$ for which $T=\sum_{a \in [l]} v_a \otimes w_a$. This completes the proof.
\end{proof}

\begin{prop}\label{prop:decomp_alg}
Let $\V$ be an $\complex$-vector space of dimension $n$, and let $\X \subseteq \V$ be a non-degenerate, irreducible, conic variety cut out by degree-2 homogeneous polynomials. Then for any $\complex$-vector space $\W$, a generic tensor $T \in \V \otimes \W$ satisfying
\ba
\setft{R}_{\X,\W}(T) < \min\{\dim(\W)+1,n-\frac{1}{n} \dim(\ker(\Phi_\X^2))\}
\ea
has a unique $(\X, \W)$-rank decomposition, and this decomposition can be obtained efficiently using the method of Theorem~\ref{thm:tensor_decomp} (i.e., the unique $(\X, \W)$-rank decomposition $T=\sum_{a \in [l]} v_a \otimes w_a$ of $T$ satisfies the property that $\{w_a : a \in [l]\}$ is linearly independent and~\eqref{eq:linintheorem} is linearly independent).
\end{prop}
\begin{proof}
A generic tensor $T \in \V \otimes \W$ of rank $\setft{R}_{\X,\W}(T)\leq \dim(\W)$ will satisfy $\setft{R}_{\X,\W}(T)=\dim(T(\W^*))$, i.e. $T(\W^*)$ is spanned by elements of $\X$. Since $T$ is generic, $T(\W^*) \subseteq \V$ is a subspace spanned by generic elements $v_1,\dots, v_l \in \X$, so by Proposition~\ref{prop:lininprop}, the set~\eqref{eq:linintheorem} is linearly independent. This completes the proof.
\end{proof}

\begin{example}
Let $\W$ be an $\field$-vector space, let $\V_1,\V_2$ be $\field$-vector spaces of dimensions $n_1, n_2$, let $\V=\V_1 \otimes \V_2$, and let $\X=\hat{\seg}(\proj \V_1 \times \proj \V_2)$ be the set of product tensors in $\V$. Then $\X$ is cut out by $2\times 2$ minors, which are degree-2 homogeneous polynomials. Note that $\dim(\ker({\Phi_\X^2}))=(n_1 n_2)^2-\binom{n_1}{2}\binom{n_2}{2}.$ By Proposition~\ref{prop:decomp_alg}, a generic tensor $T \in \V \otimes \W$ that satisfies
\ba
\setft{R}(T) < \min\{\dim(\W)+1,\frac{(n_1-1)(n_2-1)}{4}\}
\ea
has a unique $(\X,\W)$-rank decomposition, and this decomposition can be obtained efficiently using the method of Theorem~\ref{thm:tensor_decomp}.

In particular, if $\V_1=\V_2=\W=\complex^n$, then a generic tensor of rank $\setft{R}(T)\leq n$ has a unique rank decomposition, and this decomposition can be obtained efficiently using the method of Theorem~\ref{thm:tensor_decomp}; and if $\V_1=\V_2=\complex^n$, and $\W=\complex^n \otimes \complex^n$, then a generic tensor of rank $\setft{R}(T)\leq \frac{(n_1-1)(n_2-1)}{4}$ has a unique rank decomposition, and this decomposition can be obtained efficiently using the method of Theorem~\ref{thm:tensor_decomp}.
\end{example}

\comment{Ben: Can we prove that when $\X\subseteq \complex^n \otimes \complex^2$ is the set of product tensors, a generic set of $n$ vectors $v_1,\dots, v_n \in \X$ satisfies the property that
\ba
\{\Phi_\X^2(v_{a_1}\otimes v_{a_2}) : a \in [n]^{\vee 2} \setminus \Delta_n\}
\ea
is linearly independent, where $\Delta_n=\{(i,i): i \in [n]\}$? Such a statement would allow us to reproduce Jennrich's theorem.}
%\comment{Ben: The rest of this section is out of date.}
%
%
%
%
%
%
%\begin{definition}
%For $\field$-vector spaces $\V$ and $\W$ and a tensor $v \in S^2(\V \otimes \W)$, we define the $r$-\textit{aided rank} of $v$ to be the minimum number $l$ for which $v \in \hat{\Sigma}_l(\nu_2(\Sigma_r(\seg(\proj \V \times \proj \W))))$, i.e. the minimum number $l$ for which there exist tensors $v_1,\dots, v_l \in \V \otimes \W$ each of rank $\leq r$ and field elements $\alpha_1,\dots, \alpha_l\in \field$ for which
%\begin{align}
%v=\sum_{a \in [l]} \alpha_a v_a \vee v_a.
%\end{align}
%\end{definition}
%
%\begin{theorem}\label{thm:foobi_gen}
%Let $l$ and $r$ be positive integers, let $\V$ and $\W$ be vector spaces over $\field$, and let $v \in S^2(\V \otimes \W)$ be a tensor. If there exist tensors $v_1,\dots, v_l \in \V \otimes \W$ each of rank $\leq r$ for which
%\begin{align}\label{eq:unique_aided_decomp}
%v=\sum_{a \in [l]} v_a \vee v_a,
%\end{align}
%and Condition 2 from Lemma~\ref{lemma:cardoso_gen} holds, then the $r$-th aided rank of $v$ is $l$,~\eqref{eq:unique_aided_decomp} is the unique way to write $v$ as a sum of terms of the form $v_a \vee v_a$ for $v_a \in \hat{\Sigma}_r(\seg(\proj \V \times \proj \W))$ and the decomposition~\eqref{eq:unique_aided_decomp} can be obtained from $v$ in polynomial time.
%\end{theorem}
%\comment{Ben: Genericity statement? Comparison to FOOBI algorithm guarantees/smoothed analysis?}
%
%\begin{proof}
%Let $u_1,\dots, u_l \in \V \otimes \W$ be such that $v = \sum_{a=1}^l u_a \vee u_a$, which can be computed in polynomial time by a Cholesky decomposition. Let $U=(u_1,\dots, u_l)$, let $T \in S^{r+1}(\field^l)$ be a symmetric tensor satisfying~\eqref{eq:symmetric_zero_combo} (which can also be computed in polynomial time), and let $V=(v_1,\dots, v_l)$. Then there exists a unitary (or, if $\field=\real$, orthogonal) matrix $Q \in \U(\field^l)$ for which $V=UQ$, and there exist field elements $\alpha_1,\dots, \alpha_l \in \field$ for which
%\begin{align}\label{eq:T_sum}
%T=\sum_{a \in [l]} \alpha_a Q_{({:,a})}^{\vee r+1}.
%\end{align}
%If $r=1$ and $\field=\complex$, then let $\tilde{T}=\sum_{a \in [l]} \alpha_a Q_{({:,a})} Q_{({:,a})}^\t$ be the tensor $T$ viewed as a map $\V \otimes \W \rightarrow \V \otimes \W$. Then $\tilde{T}\tilde{T}^*=\sum_{a \in [l]} \abs{\alpha_a}^2 Q_{(:,a)} {Q}_{(:,a)}^*$ is a spectral decomposition of $\tilde{T}\tilde{T}^*$. By randomly choosing a symmetric tensor $T$ that satisfies~\eqref{eq:symmetric_zero_combo}, with probability one the numbers $\abs{\alpha_1}^2,\dots, \abs{\alpha_l}^2$ are non-zero and distinct, so the spectral decomposition of $\tilde{T}\tilde{T}^*$ (which is efficiently computable from $T$) uniquely determines $Q$, and hence $V$.
%
%If $r=1$ and $\field=\real$, then~\eqref{eq:T_sum} is a spectral decomposition of $T$. By randomly choosing a symmetric tensor $T$ that satisfies~\eqref{eq:symmetric_zero_combo}, with probability one the real numbers $\alpha_1,\dots, \alpha_l$ are non-zero and distinct, so the spectral decomposition is unique, and $Q$ (hence, $V$) is uniquely determined.
%
%If $r\geq 3$, then we can again choose $T$ randomly to ensure that $\alpha_1,\dots, \alpha_l$ are non-zero. In this case,~\eqref{eq:T_sum} is the unique Waring rank decomposition of $T$, and it can be obtained efficiently using e.g. Jennrich's algorithm. This allows us to obtain $Q$ and hence $V$ efficiently. This completes the proof.
%\end{proof}



%\input{genericity}


%\section{OLD Appendix}
%\begin{prop}\label{prop:lininprop}
%Let $\V$ be an $\real$-vector space of dimension $n$, and let $\X \subseteq \V$ be a conic variety with non-degenerate irreducible components that is cut out by a set of homogeneous degree-$2$ polynomials $f_1,\dots, f_{p}$. Then for any positive integer $l<\frac{n}{2}-\frac{1}{2n}\dim(\ker(\Phi_\X^2))$, and any integer $s \in [l]$, it holds that for a generic collection of vectors $v_1,\dots, v_s \in \X,v_{s+1},\dots, v_l \in \V$, the set
%\begin{align}\label{eq:lininreal}
%\{\Phi_{\X}^2(v_{a_1} \otimes v_{a_2}) : a \in [l]^{\vee 2} \setminus \Delta_s\} \subseteq \real^p
%\end{align}
%is linearly independent, where $\Delta_s=\{(i,i) : i \in [s]\} \subseteq [l]^{\vee 2}$.
%\end{prop}
%\begin{proof}
%Let $s \in [l]$ be an integer, and define the sets
%\ba
%G_1&=\{v_a \otimes v_a : a \in [l]\setminus[s]\},\\
%G_2&=\{v_{a_1} \otimes v_{a_2} : a \in [l]^{\times 2}\}.
%\ea
%Note that the set~\eqref{eq:lininreal} is linearly independent if and only if the following two properties hold:
%\begin{enumerate}
%\item For all $a \in [l]^{\vee 2}$, it holds that
%\ba\label{eq:prop1real}
%v_{a_1} \otimes v_{a_2} \notin \ker(\Phi_\X^2) + \spn(G_2 \setminus \{v_{a_1} \otimes v_{a_2}\}),
%\ea
%\item For all $a \in [l]\setminus [s]$, it holds that
%\ba
%v_a \otimes v_a \notin \ker(\Phi_\X^2) + \spn(G_1 \cup G_2 \setminus \{v_a \otimes v_a\}).
%\ea
%\end{enumerate}
%To complete the proof, we verify that Properties 1 and 2 hold for generic choices of $v_1,\dots, v_s \in \X,v_{s+1},\dots, v_l \in \V$.
%
%For vectors $v_1,\dots,v_s \in \X$ and $v_{s+1},\dots, v_l \in \V$, let
%\ba
%\U_a = \{v_a \otimes w : w \in \V\} \cup \{w \otimes v_a : w \in \V\}
%\ea
%for each $a \in [l]$. For $a \in [l]^{\vee 2}$, let
%\ba
%\U_{\hat{a}}=\spn\{ \cup_{b \in [l]\setminus \{a_1,a_2\}} \U_b\},
%\ea
%and let $\V_{\hat{a}}=\ker(\Phi_\X^2) + \U_{\hat{a}}$. Note that
%\ba
%\ker(\Phi_\X^2) + \spn(G_2 \setminus \{v_{a_1} \otimes v_{a_2}\})\subseteq \V_{\hat{a}}\subsetneq \V^{\otimes 2},
%\ea
%where the first inclusion is obvious, and the second, strict inclusion follows from
%\ba
%\dim(\V_{\hat{a}}) &\leq \dim\ker(\Phi_\X^2)+\dim(\U_{\hat{a}})\\
%			&\leq \dim\ker(\Phi_\X^2)+2 l n\\
%			&< \dim(\V^{\otimes 2}).
%\ea
%Here, the first two inequalities are obvious, and the third follows from the assumption $l<\frac{n}{2}-\frac{1}{2n}\dim(\ker(\Phi_\X^d))$. Furthermore, $\V_{\hat{a}}$ does not depend on $v_{a_1}, v_{a_2}$.
%
%Let $\X_1,\dots, \X_k$ be the irreducible components of $\X$, and for each $i,j \in [k]$ let
%\ba
%\Y_{i,j}=\{w \otimes z : w \in \X_i , z \in \X_j\}\subseteq \V^{\otimes 2}.
%\ea
%Note that $\Y_{i,j}$ is a non-degenerate, irreducible, and conic variety since $\X_i$ and $\X_j$ are. Since $\Y_{i,j}$ is non-degenerate and $\V_{\hat{a}}\subseteq \V^{\otimes 2}$ is contained in a hyperplane, it holds that $\Y_{i,j}\cap \V_{\hat{a}}\subsetneq \Y_{i,j}$ is a Zariski closed proper subset of $\Y_{i,j}$. It follows from irreducibility of $\Y_{i,j}$ that if $a_1,a_2 \in [s]$, then there is a Zariski open dense subset $\A_{i,j} \subseteq \X_i \times \X_j$ for which $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \A_{i,j}$. Since
%\ba
%\bigcup_{i,j\in [k]} \A_{i,j} \subseteq \X \times \X,
%\ea
%is a Zariski dense, constructible subset of $\X \times \X$, by [CITE AN] it contains a Zariski open dense subset $\A \subseteq \X \times \X$. Note that $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \A$. Hence, $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for a generic choice of $v_{a_1},v_{a_2}\in \X\times \X$. Similarly, if $a_1 \in [s]$ and $a_2 \in [l]\setminus [s]$, then there is a Zariski open dense subset $\B_i^{} \subseteq \X_i \times \V$ for which $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \B_{i}^{}$, so there exists a Zariski open dense subset
%\ba
%\B \subseteq \bigcup_{i\in [k]} \B_{i} \subseteq \X \times \V
%\ea
%of $\X \times \V$ for which $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \B$. In other words, $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for a generic choice of $v_{a_1} \in \X$ and $v_{a_2}\in \V$. By the same argument, if $a_1,a_2 \in [l]\setminus [s]$, then $v_{a_1}\otimes v_{a_2} \notin \V_{\hat{a}}$ for a generic choice of $v_{a_1},v_{a_2}\in \V$. In summary, we have that for any choice of $a \in [l]^{\vee 2}$, and any choice of $v_{a_3},\dots, v_{a_l}$ (each living in either $\X$ or $\V$, depending on whether $a_i \in [s]$ or $a_i\in [l]\setminus [s]$), a generic choice of $v_{a_1}, v_{a_2}$ satisfies~\eqref{eq:prop1real}. By Lemma~\ref{lemma:Zariski_dense}, we have proven that the set
%\ba
%\{(v_1,\dots, v_l)\in \X^{\times s} \times \V^{\times l-s} :\text{\eqref{eq:prop1real} holds for all}\quad a \in [l]^{\vee 2}\quad \text{with} \quad& a_1, a_2 \in [s]\}\\
%& \subseteq \X^{\times s} \times \V^{\times l-s}
%\ea
%is Zariski dense in $\X^{\times s} \times \V^{\times l-s}$. Since this set constructible, by [CITE AN] it contains a Zariski open dense subset of $\X^{\times s} \times \V^{\times l-s}$. Defining similar sets for the other cases $a_1\in [s], a_2 \in [l]\setminus[s]$ and $a_1,a_2 \in [l]\setminus[s]$, we conclude that each contains a Zariski open dense subset of $\X^{\times s} \times \V^{\times l-s}$.
%%The intersection of the three Zariski open dense subsets of $\C_{s}$, $\C_{s,l}$ and $\C_l$ is again Zariski open dense in $\X^{\times s} \times \V^{\times l-s}$.
%In summary, for each $a \in [l]^{\vee 2}$ there is a Zariski open dense subset $\C_a \subseteq \X^{\times s} \times \V^{\times l-s}$ for which \eqref{eq:prop1real} holds. It follows that
%\ba
%\C:=\bigcup_{a \in [l]^{\vee 2}} \C_a \subseteq \X^{\times s} \times \V^{\times l-s}
%\ea
%is a Zariski open dense subset for which Property 1 holds. This proves that Property 1 is satisfied for a generic choice of $v_1,\dots, v_s \in \X$ and $v_{s+1},\dots, v_l \in \V$.
%
%Property 2 is proven similarly, as follows. For $a \in [l]\setminus[s]$, let
%\ba
%\U_{\hat{a}}=\spn\{\cup_{b \in [l]\setminus \{a\}} \U_a\}
%\ea
%and
%\ba
%\V_{\hat{a}}=\ker(\Phi_\X^2) + \U_{\hat{a}},
%\ea
%and note that
%\ba
%\ker(\Phi_\X^2) + \spn(G_2 \cup G_1 \setminus \{v_{a}\otimes v_a\})\subseteq \V_{\hat{a}}\subsetneq \V^{\otimes 2},
%\ea
%by similar reasoning as above. It follows that $\V_{\hat{a}} \cap S^2(\V) \subsetneq S^2(\V)$, since $\w^2(\V) \subseteq \V_{\hat{a}}$.  Since $\V_{\hat{a}}$ does not depend on $v_a$, and
%\ba
%\Y:=\{w \otimes w : w \in \V\}\subseteq S^2(\V)
%\ea
%is an irreducible, non-degenerate, conic variety, it follows that a generic $v_a \in \V$ will satisfy $v_a \otimes v_a \notin \V_{\hat{a}}$. This proves Property 2, and completes the proof of the proposition.
%\end{proof}
%
%\begin{lemma}\label{lemma:Zariski_dense}
%Let $\Y_1, \Y_2 \subseteq \field^n$ be Zariski-closed subsets, and for each $y \in \Y_1$ let $\U_y \subseteq \Y_2$ be a Zariski open dense subset. Then
%\ba
%\bigcup_{y \in \Y_1} \{y\} \times \U_y \subseteq \Y_1 \times \Y_2
%\ea
%is Zariski dense in $\Y_1 \times \Y_2$.
%\end{lemma}
%\begin{proof}
%See the last paragraph in the proof of Theorem~7 in [CITE LOVITZ-JOHNSTON].
%\end{proof}
%
%\begin{prop}\label{prop:lininprop}
%Let $\V$ be an $\field$-vector space of dimension $n$, and let $\X \subseteq \V$ be a conic variety with non-degenerate irreducible components that is cut out by a set of homogeneous degree-$2$ polynomials $f_1,\dots, f_{p}$. Then for any positive integer
%\ba
%l<\begin{cases}
%n-\frac{1}{n}\dim(\ker(\Phi_\X^2)),& \field=\complex\\
%\frac{n}{2}-\frac{1}{2n}\dim(\ker(\Phi_\X^2)),&\field=\real
%\end{cases},
%\ea
%and any integer $s \in [l]$, it holds that for a generic collection of vectors $v_1,\dots, v_s \in \X,v_{s+1},\dots, v_l \in \V$, the set
%\begin{align}\label{eq:linin}
%\{\Phi_{\X}^2(v_{a_1} \otimes v_{a_2}) : a \in [l]^{\vee 2} \setminus \Delta_s\} \subseteq \field^p
%\end{align}
%is linearly independent, where $\Delta_s=\{(i,i) : i \in [s]\} \subseteq [l]^{\vee 2}$.
%\end{prop}
%\begin{proof}
%We prove here only the statement over the complex numbers. The proof of the statement over the real numbers is similar, and can be found in the appendix. Let $s \in [l]$ be an integer, and define the sets
%\ba
%G_1&=\{v_a \otimes v_a : a \in [l]\setminus[s]\},\\
%G_2&=\{P^{\vee}_{\V,2}(v_{a_1} \otimes v_{a_2}) : a \in [l]^{\w 2}\}.
%\ea
%Note that the set~\eqref{eq:linin} is linearly independent if and only if the following two properties hold:
%\begin{enumerate}
%\item For all $a \in [l]^{\w 2}$, it holds that
%\ba\label{eq:prop1}
%P^{\vee}_{\V,2}(v_{a_1} \otimes v_{a_2}) \notin \ker(\Phi_\X^2) + \spn(G_2 \setminus \{P^{\vee}_{\V,2}(v_{a_1} \otimes v_{a_2})\}),
%\ea
%\item For all $a \in [l]\setminus [s]$, it holds that
%\ba
%v_a \otimes v_a \notin \ker(\Phi_\X^2) + \spn(G_1 \cup G_2 \setminus \{v_a \otimes v_a\}).
%\ea
%\end{enumerate}
%To complete the proof, we verify that Properties 1 and 2 hold for generic choices of $v_1,\dots, v_s \in \X$ and $v_{s+1},\dots, v_l \in \V$.
%
%For vectors $v_1,\dots,v_s \in \X$ and $v_{s+1},\dots, v_l \in \V$, let
%\ba
%\U_a = \{P^{\vee}_{\V,2} (v_a \otimes w) : w \in \V\}
%\ea
%for each $a \in [l]$. For $a \in [l]^{\w 2}$, let
%\ba
%\U_{\hat{a}}=\spn\{ \cup_{b \in [l]\setminus \{a_1,a_2\}} \U_b\},
%\ea
%and let $\V_{\hat{a}}=S^2(\V) \cap \ker(\Phi_\X^2) + \U_{\hat{a}}$. Note that
%\ba
%S^2(\V) \cap \ker(\Phi_\X^2) + \spn(G_2 \setminus \{P^{\vee}_{\V,2}(v_{a_1} \otimes v_{a_2})\})\subseteq \V_{\hat{a}}\subsetneq S^2(\V),
%\ea
%where the first inclusion is obvious, and the second, strict inclusion follows from
%\ba
%\dim(\V_{\hat{a}}) &\leq \dim(S^2(\V) \cap \ker(\Phi_\X^2))+\dim(\U_{\hat{a}})\\
%			&\leq \dim(S^2(\V) \cap \ker(\Phi_\X^2))+l n\\
%			&< \dim(S^2(\V)).
%\ea
%Here, the first two inequalities are obvious, and the third follows from the fact that $\dim(S^2(\V) \cap \ker(\Phi_\X^2))=\dim\ker(\Phi_\X^2)-\binom{n}{2}$ and the assumption $l< n-\frac{1}{n}\dim(\ker(\Phi_\X^d))$. Furthermore, $\V_{\hat{a}}$ does not depend on $v_{a_1}, v_{a_2}$.
%
%Let $\X_1,\dots, \X_k$ be the irreducible components of $\X$, and for each $i,j \in [k]$ let
%\ba
%\Y_{i,j}=\{P^{\vee}_{\V,2} (w \otimes z) : w \in \X_i , z \in \X_j\}\subseteq S^2(\V).
%\ea
%Note that $\Y_{i,j}$ is a non-degenerate, irreducible, and conic variety since $\X_i$ and $\X_j$ are. Since $\Y_{i,j}$ is non-degenerate, it holds that $\Y_{i,j}\cap \V_{\hat{a}}\subsetneq \Y_{i,j}$ is a Zariski closed proper subset of $\Y_{i,j}$. It follows from irreducibility of $\Y_{i,j}$ that if $a_1,a_2 \in [s]$, then there is a Zariski open dense subset $\A_{i,j} \subseteq \X_i \times \X_j$ for which $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \A_{i,j}$. Since
%\ba
%\bigcup_{i,j\in [k]} \A_{i,j} \subseteq \X \times \X,
%\ea
%is a Zariski dense, constructible subset of $\X \times \X$, by [CITE AN] it contains a Zariski open dense subset $\A \subseteq \X \times \X$. Note that $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \A$. Hence, $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for a generic choice of $v_{a_1},v_{a_2}\in \X\times \X$. Similarly, if $a_1 \in [s]$ and $a_2 \in [l]\setminus [s]$, then there is a Zariski open dense subset $\B_i^{} \subseteq \X_i \times \V$ for which $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \B_{i}^{}$, so there exists a Zariski open dense subset
%\ba
%\B \subseteq \bigcup_{i\in [k]} \B_{i} \subseteq \X \times \V
%\ea
%of $\X \times \V$ for which $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for all $(v_{a_1}, v_{a_2})\in \B$. In other words, $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for a generic choice of $v_{a_1} \in \X$ and $v_{a_2}\in \V$. By the same argument, if $a_1,a_2 \in [l]\setminus [s]$, then $P^{\vee}_{\V,2}(v_{a_1}\otimes v_{a_2}) \notin \V_{\hat{a}}$ for a generic choice of $v_{a_1},v_{a_2}\in \V$. In summary, we have that for any choice of $a \in [l]^{\vee 2}$, and any choice of $v_{a_3},\dots, v_{a_l}$ (each living in either $\X$ or $\V$, depending on whether $a_i \in [s]$ or $a_i\in [l]\setminus [s]$), a generic choice of $v_{a_1}, v_{a_2}$ satisfies~\eqref{eq:prop1}. By Lemma~\ref{lemma:Zariski_dense}, we have proven that the set
%\ba
%\{(v_1,\dots, v_l)\in \X^{\times s} \times \V^{\times l-s} : \text{\eqref{eq:prop1} holds for all}\quad a \in [l]^{\vee 2}\quad \text{with} \quad &a_1, a_2 \in [s]\} \\
%&\subseteq \X^{\times s} \times \V^{\times l-s}
%\ea
%is Zariski dense in $\X^{\times s} \times \V^{\times l-s}$. Since this set constructible, by [CITE AN] it contains a Zariski open dense subset of $\X^{\times s} \times \V^{\times l-s}$. Defining similar sets for the other cases $a_1\in [s], a_2 \in [l]\setminus[s]$ and $a_1,a_2 \in [l]\setminus[s]$, we conclude that each contains a Zariski open dense subset of $\X^{\times s} \times \V^{\times l-s}$.
%%The intersection of the three Zariski open dense subsets of $\C_{s}$, $\C_{s,l}$ and $\C_l$ is again Zariski open dense in $\X^{\times s} \times \V^{\times l-s}$.
%In summary, for each $a \in [l]^{\vee 2}$ there is a Zariski open dense subset $\C_a \subseteq \X^{\times s} \times \V^{\times l-s}$ for which \eqref{eq:prop1} holds. It follows that
%\ba
%\C:=\bigcup_{a \in [l]^{\vee 2}} \C_a \subseteq \X^{\times s} \times \V^{\times l-s}
%\ea
%is a Zariski open dense subset for which Property 1 holds. This proves that Property 1 is satisfied for a generic choice of $v_1,\dots, v_s \in \X$ and $v_{s+1},\dots, v_l \in \V$.
%
%Property 2 is proven similarly, as follows. For $a \in [l]\setminus[s]$, let
%\ba
%\U_{\hat{a}}=\spn\{\cup_{b \in [l]\setminus \{a\}} \U_a\}
%\ea
%and
%\ba
%\V_{\hat{a}}=S^2(\V) \cap \ker(\Phi_\X^2) + \U_{\hat{a}},
%\ea
%and note that
%\ba
%S^2(\V) \cap \ker(\Phi_\X^2) + \spn(G_2 \cup G_1 \setminus \{v_{a}\otimes v_a\})\subseteq \V_{\hat{a}}\subsetneq S^2(\V),
%\ea
%by similar reasoning as above. Since $\V_{\hat{a}}$ does not depend on $v_a$, and
%\ba
%\Y=\{w \otimes w : w \in \V\}\subseteq S^2(\V)
%\ea
%is an irreducible, non-degenerate, conic variety, it follows that a generic $v_a \in \V$ will satisfy $v_a \otimes v_a \notin \V_{\hat{a}}$. This proves Property 2, and completes the proof of the proposition.
%\end{proof}

